AutoMerge: A Framework for Map Assembling and Smoothing in City-scale Environments

We present AutoMerge, a LiDAR data processing framework for assembling a large number of map segments into a complete map. Traditional large-scale map merging methods are fragile to incorrect data associations, and are primarily limited to working only offline. AutoMerge utilizes multi-perspective fusion and adaptive loop closure detection for accurate data associations, and it uses incremental merging to assemble large maps from individual trajectory segments given in random order and with no initial estimations. Furthermore, after assembling the segments, AutoMerge performs fine matching and pose-graph optimization to globally smooth the merged map. We demonstrate AutoMerge on both city-scale merging (120km) and campus-scale repeated merging (4.5km x 8). The experiments show that AutoMerge (i) surpasses the second- and third- best methods by 14% and 24% recall in segment retrieval, (ii) achieves comparable 3D mapping accuracy for 120 km large-scale map assembly, (iii) and it is robust to temporally-spaced revisits. To the best of our knowledge, AutoMerge is the first mapping approach that can merge hundreds of kilometers of individual segments without the aid of GPS.

==> doc/exp/analysis.tex <==
\section{Experiments}
\label{sec:experiments}
    To evaluate the map merging accuracy, we choose one public dataset \textit{KITTI}~\cite{DATASET:KITTI}, one city-scale dataset from City of Pittsburgh with $187.5km$ in total, and one campus-scale dataset within Carnegie Mellon University.
    The above datasets covers re-visit types including translation and orientation differences.
    In this section, we describe the datasets, evaluation criteria and target methods.
    
    % In this section, we compare the proposed method with the current state-of-the-art in learning-based 3D place recognition on both public and self-recorded datasets. 
    % To generate our datasets, we designed a data recording mobile platform.
    % The platform contains a LiDAR device (Velodyne-VLP 16), an inertial measurement unit (Xsense MTi $30$, $0.5^{\circ}$ error in roll/pitch, $1^{\circ}$ error in yaw, $550m$W), a mini PC (Intel NUC i7, $3.5$ GHz, $28$W) and an embedded GPU device (Nvidia Xavier, $8$G memory).
    % We trained our network model on a GPU server with a Ubuntu 18.04 system with a single Nvidia 1080Ti GPU and $64$G RAM. 
    % In the rest of this section, we will first describe both the public and self-recorded datasets.
    % Then we analyze the place recognition performance and efficiency of our methods, other state-of-the-art learning-based methods~\cite{PR:pointnetvlad,PR:LPDNet,PR:PCAN}, and non-learning based methods~\cite{Feature3D:ESF,FEATURE3D:FPFH,Feature3D:M2DP,shot}.
    % Finally, in the ablation study section, we also analyze our methods' performance under different network configurations.

    \color{red}

    \begin{table}[h]
        \centering
        \caption{Dataset frames number in training/evaluation on the four datasets.}
        \begin{tabular}{c c c c c}
        \hline
         & \textit{KITTI} & \textit{NCLT} & \textit{CAMPUS} & \textit{CITY} \\ \hline
        Train              & $13,070$ & $15,971$ & $13,830$ & $10,972$ \\ 
        Eval (test/refer)  & $3,268$  & $3,993$  & $3,458$  & $2,744$  \\ 
        \hline
        \label{table:dataset}
        \end{tabular}
    \end{table}

    \noindent \textbf{Datasets.} Our evaluation datasets include two public datasets and two self-recorded datasets:
    \begin{itemize}
        \item \textbf{KITTI} dataset, which consists of 21 trajectories generated with Velodyne-64 LiDAR scanner, around the mid-size city of Karlsruhe. 
        We use trajectory $\{1\sim 8\}$ for network training, and $\{9,10\}$ for evaluation.
        \item \textbf{Pittsburgh} dataset, which consists of 103 trajectories generated with Velodyne-32 LiDAR scanner, around the mid-size city of Karlsruhe.
        We use trajectory $\{1\sim 8\}$ for network training, and $\{9,10\}$ for evaluation.
        % We use trajectories $\{1\sim 9\}$ for network training, and $\{10,11\}$ for evaluation.
        \item \textbf{Pittsburgh dataset}, we created a City-scale dataset by mounting our data generating system on the top of a car and repeatly traversing $11km$ trajectories in the city of Pittsburgh. 
        We collected 12 trajectories, and we use trajectories $\{1\sim 10\}$ for network training, and $\{11,12\}$ for evaluation.
    \end{itemize}

    To provide training/evaluation data, we first generate the global map with all the LiDAR sequences through a traditional LiDAR odometry method~\cite{LOAM:zhang2014loam}.
    We generate the local LiDAR maps given the ground truth trajectories on each datasets, and separate them into training and evaluation datasets with shuffled index.
    The train/inference datasets are gathered individually, and we only train the network with the specific training dataset in each dataset. 
    We also prepare the corresponding position for each local map, which is necessary to calculate the position $\{S_{pos}\}$ and negative $\{S_{neg}\}$ samples for each query data $S_{q}$.
    Table~\ref{table:dataset} shows the data separation in training/evaluation on the four datasets.
    Especially, to verify the generalization ability of different methods in the evaluation step, we generate the testing data with random delta translation ($[0,2,4,6,8,...]m$ on 2D--XY plane) or delta orientation ($[0,45,90,135,...]^{\circ}$ in yaw) differences comparing the ground truth trajectory.
    
        \begin{table}[h]
        \centering
        \caption{Place recognition evaluation on different areas of \textit{CMU}}
        \begin{tabular}{c c c c c}
        \hline
         &                      \textit{Refer} & \textit{Test} & \textit{Distance} \\ \hline
        \textit{NSH}            & $1,523$ & $1,489$ & $1.5km$  \\ 
        \textit{Hamburg Hall}   & $1,830$ & $1,865$ & $1.8km$  \\ 
        \textit{Gates}          & $2,023$ & $1,948$ & $2.0km$  \\
        \hline
        \label{table:dataset_real}
        \end{tabular}
    \end{table}
    
    On the other hand, to verify the place recognition performance of two slightly different trajectories within the same area, we also record the testing/reference sequence data from different areas on the campus area as we can see in the table.~\ref{table:dataset_real}.
    The ground truth positions of testing/reference sequence queries are obtained with an offline ICP-based point cloud registration method, where each frame will take around $200\sim500ms$ with accuracy around $0.1\sim0.2m$.
    
    \bigskip
    \noindent \textbf{Methods.}
    To evaluate our approach's performance, we firstly compared it with the current state-of-the-art methods of learning-based place recognition methods, PointNetVLAD~\cite{PR:pointnetvlad}, which are re-implied from the Github\footnote{https://github.com/mikacuy/pointnetvlad}.
    For the non-learning based method, we also compare the frame-level descriptors Fast Histogram~\cite{FEATURE3D:FPFH} and M2DP~\cite{Feature3D:M2DP} from the Github\footnote{https://github.com/LiHeUA/M2DP}, and 3D keypoint-based methods ESF~\cite{Feature3D:ESF} and SHOT~\cite{shot} in the PCL library.
    For all the above approaches, we provide the dense local maps generated by our local mapping module, as shown in Section~\ref{sec:ML_SP}.
    For the all the learning-based method, we use the same data configuration on each datasets and same training epochs, and training the new network models on each of four datasets.
    To inference different real trajectories in the Campus (Table~\ref{table:dataset_real}), we use the pre-trained model on the joint Campus dataset.
    
    % Training Configurations....
    To make fair comparison with other methods, we use the same training data for all the learning based methods (FusionVLAD, PointNetVLAD), and also the same VLAD parameters for place feature aggregation.
    In the evaluation step, all the learning/non-learning methods are investigated under the same datasets.
    We also analysis different configurations of FusionVLAD: pure top-down based-, spherical based-, non-deep-fusion based- and deep-fusion based- place descriptors.
    All the analysis is depicted in the next section.
    
    %     \begin{figure*}[h]
    %     \centering
    %     \subfloat[PR-curve for Single-matching]
    %         {{\includegraphics[width=0.4\linewidth]{Imgs/exp/pr_single.pdf}}}%
    %         \qquad
    %     \subfloat[PR-curve for Sequence-matching]
    %         {{\includegraphics[width=0.4\linewidth]{Imgs/exp/pr_seq.pdf} }}%
    %     \\
    %     \subfloat[Average Precision Score for Single-matching]
    %         {{\includegraphics[width=0.4\linewidth]{Imgs/exp/auc_single.pdf}}}%
    %         \qquad
    %     \subfloat[Average Precision Score for Sequence-matching]
    %         {{\includegraphics[width=0.4\linewidth]{Imgs/exp/auc_seq.pdf}}}%
    %     \caption{\textbf{Results of single frame matching and sequence matching on \textit{NCLT} dataset under variant viewpoint differences.} 
    %     Our FusionVLAD takes advantages of both top-down/spherical view branches, and achieve more accurate place retrieval on both single/sequence-based matching modes than only replying on one branch and other methods.}
    % \label{fig:kitti_pr_auc}
    % \end{figure*}
    
    \bigskip
    \noindent \textbf{Evaluation Metrics}

    1)  Precision-Recall  Curve:We  used  the  precision-recall curve  as  a  main  evaluation  metric  [6].  As  argued  in  [6],  fora  place  recognition  system,  increasing  potential  matches  isimportant, even if a few false predictions occur [45]. We alsoe xamined the maximum F1 score [46], the harmonic mean of precision and recall, as our evaluation metric.
    
    2)  Recall  Distribution:We  would  like  to  note  that  the precision-recall  curve  may  not  fully  reveal  the  performancetoward  loop-closure  in  a  SLAM  framework.  The  spatial  andtemporal distributions of the loop-closure are essential for the SLAM,  while  the  precision-recall  curve  could  be  limited  tomeasuring the distribution of place recognition.Not all recallsshould  be  credited  equally from  the  point  of  view  of  SLAM loop-closure.  To  value  more  distributed  loop  detections,  we formulated  the  true  revisits  as  the  reference  loop  distributionand measuring Kullback–Leibler (KL) divergence against it.
    
    As  illustrated  in  Fig.  7(a),  we  constructed  a  histogram  ofthe  loop-closure  event  with  respect  to  the  translational  androtational  variance  between  a  nearest  one  in  a  map  and  aquery pose. The sample revisit events collected fromOxford2019-01-15-13-06-37contains two major groups. In thistoy example, we simulated three algorithms showing differentrecall distributions and measured KL divergence with respectto the ground-truth recall distribution. In Fig. 7(b), few loop-closures are found from the group 2 for the leftmost case. The



    \begin{figure*}[t]
        \centering
        \includegraphics[width=0.918\linewidth]{Imgs/exp/pr/orientation.pdf}
        \caption{\textbf{Localization results for different viewpoints on different datasets.}
        For each dataset, we pick one trajectory from the same domain and generate test/reference queries with different pitch angles $[5,15,30]^{\circ}$ and yaw angles $[15,45,90, 135]^{\circ}$, and then analyze the average recall for top-$N$ retrievals.
        }
        \label{fig:viewpoint_invariant}
    \end{figure*}


\newpage
\subsection{Place Recognition Results}
\label{sec:PR_results}

\subsubsection{Orientation- and Translation- Tolerance Analysis}

    We conduct experiments on four datasets to evaluate the robustness of place recognition of different methods. 
    As we can see in Fig.~\ref{fig:feature}, we calculate the average recall at top $1\%$ between reference/testing trajectories (under translation $[0,2,4,6]m$ and yaw orientation $[0,45,90,135]^{\circ}$).
    For all the non-learning based approaches, they can achieve robustly place recognition under variant orientation difference, while on the other hand, translation difference will significantly reduce their matching accuracy. 
    We can also notice that the PointNet-based method can handle translation differences locally but is sensitive to orientation differences, the matching accuracy of PointNetVLAD quickly declined as rotation differences increasing.
    Compare to the above techniques, the place descriptors of FusionVLAD are invariant to orientation-differences and can guarantee the average recall at top $1\%$ are above $80\%$ on each dataset.
   
       \begin{table}[t]
        \centering
        \caption{Average recall at top $@5$ under different areas of the campus}
        \begin{tabular}{ |c | c | c | c |}
        \hline
        Method & \textit{NSH} & \textit{Hamburg Hall} & \textit{Gates}\\ \hline
        \multicolumn{4}{|c|}{Non-Learning Methods} \\ \hline
        M2DP                & $65.38\%$ & $75.29\%$ & $72.15\%$ \\ \hline
        ESF                 & $80.14\%$ & $89.23\%$ & $86.27\%$ \\ \hline
        Fast-histogram      & $32.15\%$ & $36.94\%$ & $35.74\%$ \\ \hline
        SHOT                & $48.41\%$ & $51.58\%$ & $45.36\%$ \\ \hline
        \multicolumn{4}{|c|}{Learning Methods} \\ \hline
        PointNetVLAD        & $67.59\%$ & $72.71\%$ & $69.16\%$ \\ \hline
        Fusion (top-down)   & $80.81\%$ & $79.59\%$ & $81.36\%$ \\ \hline
        Fusion (spherical)  & $75.27\%$ & $80.24\%$ & $76.82\%$ \\ \hline
        Fusion (no deep)    & $83.86\%$ & $85.12\%$ & $86.32\%$ \\ \hline
        Fusion (deep)       & $\mathbf{89.51\%}$ & $\mathbf{92.16\%}$ & $\mathbf{88.14\%}$\\ \hline
        Fusion (without rot)& $82.73\%$ & $81.08\%$ & $83.65\%$ \\ \hline
        \end{tabular}
        \label{table:real_pr}
    \end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{Imgs/exp/analy/compare.png}
    \caption{Average precision score of sequence-matching~\cite{VPR:SeqSLAM} results on the NCLT dataset.}
    \label{fig:auc_seq}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{Imgs/exp/analy/compare.png}
    \caption{Average precision score of sequence-matching~\cite{VPR:SeqSLAM} results on the NCLT dataset.}
    \label{fig:auc_seq}
\end{figure*}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.85\linewidth]{Imgs/exp/analy/Method_compare.png}
%     \caption{Average precision score of sequence-matching~\cite{VPR:SeqSLAM} results on the NCLT dataset.}
%     \label{fig:auc_seq}
% \end{figure*}


    \newpage    
    Table.\ref{table:ar_1} further provides the average recall at top $@5$, we can see that on all the four datasets.
    Here Fusion (top-down) and Fusion (spherical) indicates the network with only one perspective.
    As we mentioned in Section.~\ref{sec:loss}, Fusion (no deep) means FusionVLAD network but only with fusion-branch loss in the training procedure, and Fusion (deep) is with all the three branches.
    Fusion (without rot) means the training procedure without `rotation loss' metric.  
    FusionVLAD can achieve more accurate place retrieval with average recall above $85\%$.
    Table.\ref{table:real_pr} shows the place recognition performance on the datasets of~\ref{table:dataset_real}, and all the learning methods use the pre-trained model on the Campus datasets.

    \begin{figure}[t]
        \centering
        \includegraphics[width=\linewidth]{Imgs/exp/analy/Error_dist.png}
        \caption{PR-curve for Single-matching on NCLT datasets.}
        \label{fig:pr_single}
    \end{figure}
    
    % \begin{figure*}[t]
    %     \centering
    %     \includegraphics[width=\linewidth]{Imgs/exp/analy/Distribution_analysis.png}
    %     \caption{Average precision score of single-matching results on the NCLT dataset.}
    %     \label{fig:auc_single}
    % \end{figure*}



\newpage
\subsection{Adaptive Loop Closure Detection}
\label{sec:ada_loop}

\newpage
analysis

\newpage
analysis

\newpage
analysis

\newpage 
add
\newpage
\subsection{Incremental Clustering}
\label{sec:im_cluster}

    \begin{figure}[t]
    	\centering
        	\includegraphics[width=\linewidth]{Imgs/exp/cluster.png}
    	\caption{\textbf{Incremental clustering.}
    	}
    	\label{fig:spectral}
    \end{figure}

    \newpage

    \begin{figure}[t]
    	\centering
        	\includegraphics[width=\linewidth]{Imgs/exp/cluster.png}
    	\caption{\textbf{Incremental clustering.}
    	}
    	\label{fig:spectral}
    \end{figure}

\newpage
analysis


\newpage
\subsection{Time and Storage Analysis}
    \label{sec:exp_runtime}
    In Table.~\ref{table:time_efficiency}, we analysis the time and memory usage of our FusionVLAD and other methods.
    Compared with PointNetVLAD, our method consumes about $31\%$ GPU memory for training and takes about $20\%$ time for extracting place descriptor for a point cloud.
    While comparing to non-learning method, FusionVLAD is more robust and efficient.
    In the inference step, the multi-view generation step will consume $100ms$ on the NUC i7 computer.
    FusionVLAD also only requires $10ms$ and $37Mb$ on the GPU device or $87ms$ on a CPU device.
    which make it easy to imply in the Nvidia embedded system (Nvidia Jetson TX2, or Xavier) or the NUC computer, and suitable for low cost robot systems in long-term SLAM or navigation tasks.
    

    \begin{figure}[t]
        \centering
        \includegraphics[width=\linewidth]{Imgs/exp/compute/oritention_diff.pdf}
        \caption{\textbf{Orientation estimation on our two datasets.}
        For each dataset, we manually set the orientation difference between testing and reference queries with a default yaw offset of $\mathcal{N}\sim(0,90^\circ)$, and analyze the relative orientation estimation of the PSE module.}
        \label{fig:exp_orientation}
    \end{figure}

    
    \begin{table}[t]
        \centering
        \caption{Comparison of time, GPU memory (Megabyte), and feature size requirements of different methods.
        }
        \begin{tabular}{ |c | c | c | c |}
        \hline
        Method      & GPU (MB)   & Time (ms) & Feature Size  \\ \hline
        \multicolumn{4}{|c|}{Non-Learning Methods} \\ \hline
        \textit{M2DP}  &  $-$   & $164.05$     & $192$    \\  \hline
        \textit{ESF}   &  $-$   & $14.56$      & $640$     \\  \hline
        \textit{Fast-histogram} & $-$ & $1.47$ & $80$    \\  \hline
        \textit{SHOT}  &  $-$   & $14.74$      & $352$    \\  \hline
        \multicolumn{4}{|c|}{Learning Methods} \\ \hline
        \textit{PointNetVLAD} & $7,711$ & $55.00$ & $256$ \\ \hline 
        \textit{FusionVLAD} & $2,459$ & $10.00$ & $256$ \\ \hline
        \end{tabular}
        \label{table:time_efficiency}
    \end{table}


==> doc_review/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/Peng.png}}]
    {Peng Yin} received his Bachelor's degree from Harbin Institute of Technology, Harbin, China, in 2013, and his Ph.D. degree from the University of Chinese Academy of Sciences, Beijing, in 2018.
    He is a Post-doctoral researcher with the Robotics Institute at Carnegie Mellon University, Pittsburgh, USA.
    His research interests include LiDAR SLAM, Place Recognition, 3D Perception, and Reinforcement Learning. Dr. Yin has served as a Reviewer for several IEEE Conferences ICRA, IROS, ACC, RSS.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/shiqi.png}}]
    {Shiqi Zhao} received his Bachelor's degree from Dalian University of Technology, Dalian, China, in 2018, and his Master's degree from the University of California San Diego, U.S., in 2020.
    He is currently working as an intern at the Robotics Institute at Carnegie Mellon University.
    His research interests include Place Recognition, 3D Perception, and Deep Learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/haowen.png}}]
    {Haowen Lai} received his B.E. degree in control science and engineering from Tongji University, Shanghai, China, in 2019. He is currently pursuing an M.S. degree from Tsinghua University in Beijing, China. His research mainly covers 3D localization and perception, SLAM, Place Recognition, and their application in robotics. 
    He is trying to apply computer vision and machine learning techniques to robotics so as to make robots more intelligent in understanding the environment.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/ruohai.png}}]
    {Ruohai Ge} received his B.S. degree in Electrical Engineering with a double major in Robotics from Carnegie Mellon University in 2016. He is currently working on a Master's degree in Robotics within the Robotics Institute at Carnegie Mellon University. His research interests include visual localization and robotic related software infrastructure. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/ruijief.png}}]
    {Ruijie Fu} was born in Xi’an, China in 1999. She received her Bachelor of Science degree in Mathematics in 2020 from Carnegie Mellon University, Pittsburgh, PA, USA, where she is currently working toward an M.S. degree in robotics. Her research interests include differential geometry and robot localization.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/ivan.png}}]
    {Ivan Cisneros} received his B.S. in Electrical Engineering with a minor in Computer Science from Harvard University in 2016.
    He worked full-time at NASA-JPL on several flight projects for 3 years before starting his graduate studies at Carnegie Mellon University. He is currently working on a Master's degree in Robotics at the Robotics Institute at CMU.
    His research interests include SLAM, visual localization, 3D Perception, and Deep Learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/zhang_ji.png}}]
    {Ji Zhang} received his Ph.D. in Robotics from Carnegie Mellon University in 2017.
    Ji Zhang is a Systems Scientist at the Robotics Institute at Carnegie Mellon University, where he leads in the development of a series of autonomous navigation algorithms. His work was ranked \#1 on the odometry leaderboard of KITTI Vision Benchmark between 2014 and 2021. 
    He founded Kaarta, Inc, a CMU spin-off commercializing 3D mapping \& modeling technologies, and stayed with the company for 4 years as chief scientist.
    His research interests are in robotic navigation, spanning localization, mapping, planning, and exploration.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/howie.png}}]
    {Howie Choset} received his B.S. Eng. degree in computer science and his B.S. Econ. degree in entrepreneurial management from the University of Pennsylvania (Wharton), Philadelphia, PA, USA, in 1990. He received M.S. and Ph.D. degrees in mechanical engineering from California Institute of Technology (Caltech), Pasadena, CA, USA, in 1991 and 1996, respectively.
    He is currently a Professor of Robotics at Carnegie Mellon University, Pittsburgh, PA, USA. His research group reduces complicated high dimensional problems found in robotics to low-dimensional simpler ones for design, analysis, and planning. 
    % Prof. Choset was elected as one of the top 100 innovators in the world under 35, by the MIT Technology Review, in 2002. In 2014, Popular Science selected his medical robotics work as the Best of What’s New in Health Care. 
\end{IEEEbiography}

\vspace{-1cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/basti.png}}]
    {Sebastian Scherer} received his B.S. in Computer Science, M.S. and Ph.D. in Robotics from CMU in 2004, 2007, and 2010. 
    Sebastian Scherer is an Associate Research Professor at the Robotics Institute at Carnegie Mellon University. His research focuses on enabling autonomy for unmanned rotorcraft to operate at low altitude in cluttered environments. He is a Siebel scholar and a recipient of multiple paper awards and nominations, including AIAA@Infotech 2010 and FSR 2013. His research has been covered by the national and internal press including IEEE Spectrum, the New Scientist, Wired, der Spiegel, and the WSJ. 
\end{IEEEbiography}


==> doc_review/conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}
    In this paper\added{,} we proposed AutoMerge, the first real-world automatic merging system for large-scale 3D mapping.
    \deleted{Without using the initial positions of segments in the global frame, }AutoMerge can automatically detect the relative overlaps between segments due to its viewpoint-invariant place recognition ability without using the initial positions of segments in the global frame.
    \replaced{Despite}{In spite of} the complicated \replaced{city}{cite}-scale environments and similar-looking 3D areas under different scenarios, AutoMerge provides highly accurate data \replaced{associated}{association} with our adaptive loop closure detection module.
    Finally, \deleted{by using the incremental merging module, }AutoMerge can successfully merge sub-segments \deleted{that are }given in non-sequential order\added{ using the incremental merging module}.
    The above properties make AutoMerge suitable to merge large-scale maps, such as \replaced{city}{cite}-scale, campus-scale, and subterranean environments.
    
    The results on both public and self-recorded datasets show \added{that }our place retrieval ability notably outperforms all \deleted{of the }state-of-the-art methods in 3D loop closure detection.
    Because of its high recall rates and \deleted{its }incremental merging ability, AutoMerge seems like a promising method to use on various real-world datasets.
    Our method can work with limited computational resources and storage space, making it extremely suitable for low-cost robots in large-scale map merging tasks.
    In future works, we will target the current limitations of our method and make this code publicly available.

==> doc_review/discuss.tex <==
\section{Discussion \& Limitations}
\label{sec:discussion}
    As shown in the above analysis, AutoMerge can provide robust map merging for \deleted{both }city-scale and campus-scale environments without any initial estimation.
    This framework can provide \deleted{both }offline/online merging for single- and multi-agent systems\deleted{,} while ignoring viewpoint and temporal differences\deleted{ that are} common in real-world mapping scenarios.
    However, AutoMerge also has the following limitations.
    
    AutoMerge heavily utilizes generated dense local maps. Thus, the place recognition accuracy is determined by the stability of these local maps.
    As shown in Fig.~\ref{fig:merge_noise}, when the agent is moving too fast (red circle) or there exist too many dynamic objects (yellow circle), the noise and sparse local maps negatively impact the merging procedure.
    Such observations will introduce uncertainty in the extracted place descriptor and indirectly affect the final merging performance.
    
    Besides the noise and sparsity, the extracted place descriptor is also sensitive to confined environments.
    In indoor areas, tunnels, and underground environments\added{,} the generated LiDAR map is constrained within a relatively small space compared to outdoor environments.
    In these cases, distinguishable features cannot be easily extracted from either point-based or spherical projection-based data formats.
    To obtain rich geometries, point meshlization could be a potential solution.

    Additionally, the adaptive loop closure detection \replaced{relies}{is} highly\deleted{ reliant} on the sequence matching results, and subsequently, its sequence searching process is the most time-consuming part of AutoMerge. Since the main procedure in sequence matching is the brute-force searching operation, a CUDA-enhanced sequence matching mechanism can further improve searching efficiency, as mentioned in~\cite{cuda_seqslam}.
    
    AutoMerge cannot handle trajectories with limited overlap.
    Since high merging accuracy is our primary goal, only high confidence overlaps are selected as loop closure candidates.
    The major drawback of this mechanism is missed loop closures in trajectories with minimum overlap. These cases \deleted{are }usually \replaced{occur}{encountered} at crossroads where neighbor trajectories only have $1\sim 2$ matched keyframes.
    However, from the standpoint of large-scale merging performance, this principle is necessary since we need to detect potential overlaps within hundreds of kilometers of trajectories; in such a scenario, several wrong short-range matches will crash the entire system.

    \added{Furthermore, AutoMerge cannot handle degradation areas without GPS assistance, such as highways, long tunnels, etc.
    The challenges come from two-folds:
    1) the non-distinguishable place descriptor will reduce the overlap detection accuracy in such areas.
    2) the degradation areas will also be challenging for the odometry estimation, which indirectly affects the key-frame extraction (given that the distance between key-frames is based on the odometry estimation).
    A potential solution is to combine texture-rich visual features into the place descriptor engine as stated in our previous work~\cite{adafusion} and add fuse visual/wheel odometry into the LiDAR SLAM system to reduce the odometry drift in the degradation area.
    Enable AutoMerge under the degradation case is also an inspiring trend; we would like to leave it to our further work.}

    \replaced{In general}{Finally}, the map merging ability of AutoMerge can be further extended with other types of \replaced{sensors, such as new types of LiDAR sensors (solid-state LiDAR) and cameras (omnidirectional cameras) }{sensors (e.g., new types of LiDAR or visual sensors) and place descriptor extraction methods}.
    Because AutoMerge provides a map merging framework, any existing modules within AutoMerge can be replaced to fit the specific properties of other sensors\added{ and network structures}.

    \added{Finally, data compression can also be a potential research extension for AutoMerge.
    In our experiment, we notice that AutoMerge can use low-resolution ($0.5m$ in voxel) point clouds for roughly large-scale map merging.
    Given the current research progress on point cloud compression~\cite{wiesmann2021ral}, we notice that will be a potential chance for large-scale map sharing under low-bandwidth communication, especially for service robotics, last-mile delivery and autonomous driving.
    Another potential direction is to combine AutoMerge with the increasing requirements of the low-cost visual localization system~\cite{i3dloc,panek2022meshloc}, where AutoMerge can provide the reference meshes/semantics for accurate visual navigation.}

==> doc_review/exp/analysis.tex <==
\section{Experiments}
\label{sec:experiments}
    To evaluate the map merging accuracy, we choose one public dataset \textit{KITTI}~\cite{DATASET:KITTI}, one city-scale dataset from City of Pittsburgh with $187.5km$ in total, and one campus-scale dataset within Carnegie Mellon University.
    The above datasets covers re-visit types including translation and orientation differences.
    In this section, we describe the datasets, evaluation criteria and target methods.
    
    % In this section, we compare the proposed method with the current state-of-the-art in learning-based 3D place recognition on both public and self-recorded datasets. 
    % To generate our datasets, we designed a data recording mobile platform.
    % The platform contains a LiDAR device (Velodyne-VLP 16), an inertial measurement unit (Xsense MTi $30$, $0.5^{\circ}$ error in roll/pitch, $1^{\circ}$ error in yaw, $550m$W), a mini PC (Intel NUC i7, $3.5$ GHz, $28$W) and an embedded GPU device (Nvidia Xavier, $8$G memory).
    % We trained our network model on a GPU server with a Ubuntu 18.04 system with a single Nvidia 1080Ti GPU and $64$G RAM. 
    % In the rest of this section, we will first describe both the public and self-recorded datasets.
    % Then we analyze the place recognition performance and efficiency of our methods, other state-of-the-art learning-based methods~\cite{PR:pointnetvlad,PR:LPDNet,PR:PCAN}, and non-learning based methods~\cite{Feature3D:ESF,FEATURE3D:FPFH,Feature3D:M2DP,shot}.
    % Finally, in the ablation study section, we also analyze our methods' performance under different network configurations.

    \color{red}

    \begin{table}[h]
        \centering
        \caption{Dataset frames number in training/evaluation on the four datasets.}
        \begin{tabular}{c c c c c}
        \hline
         & \textit{KITTI} & \textit{NCLT} & \textit{CAMPUS} & \textit{CITY} \\ \hline
        Train              & $13,070$ & $15,971$ & $13,830$ & $10,972$ \\ 
        Eval (test/refer)  & $3,268$  & $3,993$  & $3,458$  & $2,744$  \\ 
        \hline
        \label{table:dataset}
        \end{tabular}
    \end{table}

    \noindent \textbf{Datasets.} Our evaluation datasets include two public datasets and two self-recorded datasets:
    \begin{itemize}
        \item \textbf{KITTI} dataset, which consists of 21 trajectories generated with Velodyne-64 LiDAR scanner, around the mid-size city of Karlsruhe. 
        We use trajectory $\{1\sim 8\}$ for network training, and $\{9,10\}$ for evaluation.
        \item \textbf{Pittsburgh} dataset, which consists of 103 trajectories generated with Velodyne-32 LiDAR scanner, around the mid-size city of Karlsruhe.
        We use trajectory $\{1\sim 8\}$ for network training, and $\{9,10\}$ for evaluation.
        % We use trajectories $\{1\sim 9\}$ for network training, and $\{10,11\}$ for evaluation.
        \item \textbf{Pittsburgh dataset}, we created a City-scale dataset by mounting our data generating system on the top of a car and repeatly traversing $11km$ trajectories in the city of Pittsburgh. 
        We collected 12 trajectories, and we use trajectories $\{1\sim 10\}$ for network training, and $\{11,12\}$ for evaluation.
    \end{itemize}

    To provide training/evaluation data, we first generate the global map with all the LiDAR sequences through a traditional LiDAR odometry method~\cite{LOAM:zhang2014loam}.
    We generate the local LiDAR maps given the ground truth trajectories on each datasets, and separate them into training and evaluation datasets with shuffled index.
    The train/inference datasets are gathered individually, and we only train the network with the specific training dataset in each dataset. 
    We also prepare the corresponding position for each local map, which is necessary to calculate the position $\{S_{pos}\}$ and negative $\{S_{neg}\}$ samples for each query data $S_{q}$.
    Table~\ref{table:dataset} shows the data separation in training/evaluation on the four datasets.
    Especially, to verify the generalization ability of different methods in the evaluation step, we generate the testing data with random delta translation ($[0,2,4,6,8,...]m$ on 2D--XY plane) or delta orientation ($[0,45,90,135,...]^{\circ}$ in yaw) differences comparing the ground truth trajectory.
    
        \begin{table}[h]
        \centering
        \caption{Place recognition evaluation on different areas of \textit{CMU}}
        \begin{tabular}{c c c c c}
        \hline
         &                      \textit{Refer} & \textit{Test} & \textit{Distance} \\ \hline
        \textit{NSH}            & $1,523$ & $1,489$ & $1.5km$  \\ 
        \textit{Hamburg Hall}   & $1,830$ & $1,865$ & $1.8km$  \\ 
        \textit{Gates}          & $2,023$ & $1,948$ & $2.0km$  \\
        \hline
        \label{table:dataset_real}
        \end{tabular}
    \end{table}
    
    On the other hand, to verify the place recognition performance of two slightly different trajectories within the same area, we also record the testing/reference sequence data from different areas on the campus area as we can see in the table.~\ref{table:dataset_real}.
    The ground truth positions of testing/reference sequence queries are obtained with an offline ICP-based point cloud registration method, where each frame will take around $200\sim500ms$ with accuracy around $0.1\sim0.2m$.
    
    \bigskip
    \noindent \textbf{Methods.}
    To evaluate our approach's performance, we firstly compared it with the current state-of-the-art methods of learning-based place recognition methods, PointNetVLAD~\cite{PR:pointnetvlad}, which are re-implied from the Github\footnote{https://github.com/mikacuy/pointnetvlad}.
    For the non-learning based method, we also compare the frame-level descriptors Fast Histogram~\cite{FEATURE3D:FPFH} and M2DP~\cite{Feature3D:M2DP} from the Github\footnote{https://github.com/LiHeUA/M2DP}, and 3D keypoint-based methods ESF~\cite{Feature3D:ESF} and SHOT~\cite{shot} in the PCL library.
    For all the above approaches, we provide the dense local maps generated by our local mapping module, as shown in Section~\ref{sec:ML_SP}.
    For the all the learning-based method, we use the same data configuration on each datasets and same training epochs, and training the new network models on each of four datasets.
    To inference different real trajectories in the Campus (Table~\ref{table:dataset_real}), we use the pre-trained model on the joint Campus dataset.
    
    % Training Configurations....
    To make fair comparison with other methods, we use the same training data for all the learning based methods (FusionVLAD, PointNetVLAD), and also the same VLAD parameters for place feature aggregation.
    In the evaluation step, all the learning/non-learning methods are investigated under the same datasets.
    We also analysis different configurations of FusionVLAD: pure top-down based-, spherical based-, non-deep-fusion based- and deep-fusion based- place descriptors.
    All the analysis is depicted in the next section.
    
    %     \begin{figure*}[h]
    %     \centering
    %     \subfloat[PR-curve for Single-matching]
    %         {{\includegraphics[width=0.4\linewidth]{Imgs/exp/pr_single.pdf}}}%
    %         \qquad
    %     \subfloat[PR-curve for Sequence-matching]
    %         {{\includegraphics[width=0.4\linewidth]{Imgs/exp/pr_seq.pdf} }}%
    %     \\
    %     \subfloat[Average Precision Score for Single-matching]
    %         {{\includegraphics[width=0.4\linewidth]{Imgs/exp/auc_single.pdf}}}%
    %         \qquad
    %     \subfloat[Average Precision Score for Sequence-matching]
    %         {{\includegraphics[width=0.4\linewidth]{Imgs/exp/auc_seq.pdf}}}%
    %     \caption{\textbf{Results of single frame matching and sequence matching on \textit{NCLT} dataset under variant viewpoint differences.} 
    %     Our FusionVLAD takes advantages of both top-down/spherical view branches, and achieve more accurate place retrieval on both single/sequence-based matching modes than only replying on one branch and other methods.}
    % \label{fig:kitti_pr_auc}
    % \end{figure*}
    
    \bigskip
    \noindent \textbf{Evaluation Metrics}

    1)  Precision-Recall  Curve:We  used  the  precision-recall curve  as  a  main  evaluation  metric  [6].  As  argued  in  [6],  fora  place  recognition  system,  increasing  potential  matches  isimportant, even if a few false predictions occur [45]. We alsoe xamined the maximum F1 score [46], the harmonic mean of precision and recall, as our evaluation metric.
    
    2)  Recall  Distribution:We  would  like  to  note  that  the precision-recall  curve  may  not  fully  reveal  the  performancetoward  loop-closure  in  a  SLAM  framework.  The  spatial  andtemporal distributions of the loop-closure are essential for the SLAM,  while  the  precision-recall  curve  could  be  limited  tomeasuring the distribution of place recognition.Not all recallsshould  be  credited  equally from  the  point  of  view  of  SLAM loop-closure.  To  value  more  distributed  loop  detections,  we formulated  the  true  revisits  as  the  reference  loop  distributionand measuring Kullback–Leibler (KL) divergence against it.
    
    As  illustrated  in  Fig.  7(a),  we  constructed  a  histogram  ofthe  loop-closure  event  with  respect  to  the  translational  androtational  variance  between  a  nearest  one  in  a  map  and  aquery pose. The sample revisit events collected fromOxford2019-01-15-13-06-37contains two major groups. In thistoy example, we simulated three algorithms showing differentrecall distributions and measured KL divergence with respectto the ground-truth recall distribution. In Fig. 7(b), few loop-closures are found from the group 2 for the leftmost case. The



    \begin{figure*}[t]
        \centering
        \includegraphics[width=0.918\linewidth]{Imgs/exp/pr/orientation.pdf}
        \caption{\textbf{Localization results for different viewpoints on different datasets.}
        For each dataset, we pick one trajectory from the same domain and generate test/reference queries with different pitch angles $[5,15,30]^{\circ}$ and yaw angles $[15,45,90, 135]^{\circ}$, and then analyze the average recall for top-$N$ retrievals.
        }
        \label{fig:viewpoint_invariant}
    \end{figure*}


\newpage
\subsection{Place Recognition Results}
\label{sec:PR_results}

\subsubsection{Orientation- and Translation- Tolerance Analysis}

    We conduct experiments on four datasets to evaluate the robustness of place recognition of different methods. 
    As we can see in Fig.~\ref{fig:feature}, we calculate the average recall at top $1\%$ between reference/testing trajectories (under translation $[0,2,4,6]m$ and yaw orientation $[0,45,90,135]^{\circ}$).
    For all the non-learning based approaches, they can achieve robustly place recognition under variant orientation difference, while on the other hand, translation difference will significantly reduce their matching accuracy. 
    We can also notice that the PointNet-based method can handle translation differences locally but is sensitive to orientation differences, the matching accuracy of PointNetVLAD quickly declined as rotation differences increasing.
    Compare to the above techniques, the place descriptors of FusionVLAD are invariant to orientation-differences and can guarantee the average recall at top $1\%$ are above $80\%$ on each dataset.
   
       \begin{table}[t]
        \centering
        \caption{Average recall at top $@5$ under different areas of the campus}
        \begin{tabular}{ |c | c | c | c |}
        \hline
        Method & \textit{NSH} & \textit{Hamburg Hall} & \textit{Gates}\\ \hline
        \multicolumn{4}{|c|}{Non-Learning Methods} \\ \hline
        M2DP                & $65.38\%$ & $75.29\%$ & $72.15\%$ \\ \hline
        ESF                 & $80.14\%$ & $89.23\%$ & $86.27\%$ \\ \hline
        Fast-histogram      & $32.15\%$ & $36.94\%$ & $35.74\%$ \\ \hline
        SHOT                & $48.41\%$ & $51.58\%$ & $45.36\%$ \\ \hline
        \multicolumn{4}{|c|}{Learning Methods} \\ \hline
        PointNetVLAD        & $67.59\%$ & $72.71\%$ & $69.16\%$ \\ \hline
        Fusion (top-down)   & $80.81\%$ & $79.59\%$ & $81.36\%$ \\ \hline
        Fusion (spherical)  & $75.27\%$ & $80.24\%$ & $76.82\%$ \\ \hline
        Fusion (no deep)    & $83.86\%$ & $85.12\%$ & $86.32\%$ \\ \hline
        Fusion (deep)       & $\mathbf{89.51\%}$ & $\mathbf{92.16\%}$ & $\mathbf{88.14\%}$\\ \hline
        Fusion (without rot)& $82.73\%$ & $81.08\%$ & $83.65\%$ \\ \hline
        \end{tabular}
        \label{table:real_pr}
    \end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{Imgs/exp/analy/compare.png}
    \caption{Average precision score of sequence-matching~\cite{VPR:SeqSLAM} results on the NCLT dataset.}
    \label{fig:auc_seq}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{Imgs/exp/analy/compare.png}
    \caption{Average precision score of sequence-matching~\cite{VPR:SeqSLAM} results on the NCLT dataset.}
    \label{fig:auc_seq}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{Imgs/exp/analy/Method_compare.png}
    \caption{Average precision score of sequence-matching~\cite{VPR:SeqSLAM} results on the NCLT dataset.}
    \label{fig:auc_seq}
\end{figure*}


    \newpage    
    Table.\ref{table:ar_1} further provides the average recall at top $@5$, we can see that on all the four datasets.
    Here Fusion (top-down) and Fusion (spherical) indicates the network with only one perspective.
    As we mentioned in Section.~\ref{sec:loss}, Fusion (no deep) means FusionVLAD network but only with fusion-branch loss in the training procedure, and Fusion (deep) is with all the three branches.
    Fusion (without rot) means the training procedure without `rotation loss' metric.  
    FusionVLAD can achieve more accurate place retrieval with average recall above $85\%$.
    Table.\ref{table:real_pr} shows the place recognition performance on the datasets of~\ref{table:dataset_real}, and all the learning methods use the pre-trained model on the Campus datasets.

    \begin{figure}[t]
        \centering
        \includegraphics[width=\linewidth]{Imgs/exp/analy/Error_dist.png}
        \caption{PR-curve for Single-matching on NCLT datasets.}
        \label{fig:pr_single}
    \end{figure}
    
    % \begin{figure*}[t]
    %     \centering
    %     \includegraphics[width=\linewidth]{Imgs/exp/analy/Distribution_analysis.png}
    %     \caption{Average precision score of single-matching results on the NCLT dataset.}
    %     \label{fig:auc_single}
    % \end{figure*}



\newpage
\subsection{Adaptive Loop Closure Detection}
\label{sec:ada_loop}

\newpage
analysis

\newpage
analysis

\newpage
analysis

\newpage 
add
\newpage
\subsection{Incremental Clustering}
\label{sec:im_cluster}

    \begin{figure}[t]
    	\centering
        	\includegraphics[width=\linewidth]{Imgs/exp/cluster.png}
    	\caption{\textbf{Incremental clustering.}
    	}
    	\label{fig:spectral}
    \end{figure}

    \newpage

    \begin{figure}[t]
    	\centering
        	\includegraphics[width=\linewidth]{Imgs/exp/cluster.png}
    	\caption{\textbf{Incremental clustering.}
    	}
    	\label{fig:spectral}
    \end{figure}

\newpage
analysis


\newpage
\subsection{Time and Storage Analysis}
    \label{sec:exp_runtime}
    In Table.~\ref{table:time_efficiency}, we analysis the time and memory usage of our FusionVLAD and other methods.
    Compared with PointNetVLAD, our method consumes about $31\%$ GPU memory for training and takes about $20\%$ time for extracting place descriptor for a point cloud.
    While comparing to non-learning method, FusionVLAD is more robust and efficient.
    In the inference step, the multi-view generation step will consume $100ms$ on the NUC i7 computer.
    FusionVLAD also only requires $10ms$ and $37Mb$ on the GPU device or $87ms$ on a CPU device.
    which make it easy to imply in the Nvidia embedded system (Nvidia Jetson TX2, or Xavier) or the NUC computer, and suitable for low cost robot systems in long-term SLAM or navigation tasks.
    

    \begin{figure}[t]
        \centering
        \includegraphics[width=\linewidth]{Imgs/exp/compute/oritention_diff.pdf}
        \caption{\textbf{Orientation estimation on our two datasets.}
        For each dataset, we manually set the orientation difference between testing and reference queries with a default yaw offset of $\mathcal{N}\sim(0,90^\circ)$, and analyze the relative orientation estimation of the PSE module.}
        \label{fig:exp_orientation}
    \end{figure}

    
    \begin{table}[t]
        \centering
        \caption{Comparison of time, GPU memory (Megabyte), and feature size requirements of different methods.
        }
        \begin{tabular}{ |c | c | c | c |}
        \hline
        Method      & GPU (MB)   & Time (ms) & Feature Size  \\ \hline
        \multicolumn{4}{|c|}{Non-Learning Methods} \\ \hline
        \textit{M2DP}  &  $-$   & $164.05$     & $192$    \\  \hline
        \textit{ESF}   &  $-$   & $14.56$      & $640$     \\  \hline
        \textit{Fast-histogram} & $-$ & $1.47$ & $80$    \\  \hline
        \textit{SHOT}  &  $-$   & $14.74$      & $352$    \\  \hline
        \multicolumn{4}{|c|}{Learning Methods} \\ \hline
        \textit{PointNetVLAD} & $7,711$ & $55.00$ & $256$ \\ \hline 
        \textit{FusionVLAD} & $2,459$ & $10.00$ & $256$ \\ \hline
        \end{tabular}
        \label{table:time_efficiency}
    \end{table}


==> doc_review/exp/compute.tex <==

\subsection{Time and Storage Analysis}
    \label{sec:exp_runtime}
    
    In this section, we compare the proposed method with the current state-of-the-art in learning-based 3D place recognition on both public and self-recorded datasets. 
    To generate our datasets, we designed a data recording mobile platform.
    All the experiments are conducted on an Ubuntu 18.04 system with Nvidia RTX2060 GPU cards and $64$G RAM.
    Table.~\ref{table:time_efficiency} shows the memory usage, inference time\added{,} and feature size for all the compared place descriptor methods. 
    Compared with other methods, AutoMerge utilizes less GPU memory and has lower inference time with small storage requirements, which indicates that AutoMerge can be easily combined with current embedded systems.
    
    We further investigate the time efficiency of the incremental merging procedure; in  Fig.~\ref{fig:time_analsis} we analyze the time usage during the incremental map merging for the \textit{Pittsburgh} dataset.
    As we can see, with the AutoMerge framework, both feature extraction and map optimization are efficient, but data association is time-consuming.
    AutoMerge can infer a $5\sim 10 km$ trajectory within $2s$, and optimize the global map within $0.5s$, but data association time ranges from $4s$ to $290s$.
    This is mainly due to the computational complexity of sequence matching~\cite{2012SeqSLAM}, which is $O(n^2)$ where $n$ is the number of keyframes.
    The complexity increases with the reference map scale.
    Since the main procedure in sequence matching is the matrix multiplication operation, one solution for this problem is to apply CUDA-based sequence matching to reduce complexity.

==> doc_review/exp/merge_campus.tex <==
\subsubsection{Merging on \textit{Campus}}
\label{sec:cmu_merge}

For the \textit{Campus} dataset, we consider map merging in multi-session scenarios, where each area will be revisited multiple times, with the goal being achieving long-term autonomy.
We chose $8$ scenarios from the campus areas with sufficient temporal differences (from $3\sim 5$ days), and each trajectory is revisited $8$ times with different traversal directions (forward/reverse) and illumination (day/night) conditions.
As shown in Fig.~\ref{fig:offline_campus}, for each segment, we use a one-time visit as the reference map, and the rest of the visits as new queries.
AutoMerge can automatically detect the loop closures between query and test keyframes through our invariant place descriptor and adaptive detection mechanism.
Without any initial estimation, all segments over the same path are able to be transformed into one consistent map.
The final refinements are conducted by Iterative Closet Point (ICP).
However, due to dynamic objects and other sources of noise that occur in multiple visits, noisy merging will occur, especially in confined areas.
This problem is most prevalent in segments $7$ and $8$, which contain lots of dynamic walking pedestrians within confined campus areas, and consequently the merged global map contains lots of merging noise.
Improvements can be made by excluding dynamic objects and using accurate General-ICP~\cite{GICP}, but those methods require additional computation cost.



To better examine the merging performance in multi-session revisits, we visualize the data association for segment $1$ as shown in Fig.~\ref{fig:merge_cmu_trj1}.
Different segments are drawn with different colors, and red links indicate the inner connections between them.
To simplify the visualization, we did not draw all of the links between all of the pairs.
The omnidirectional camera shows the appearances of the same area under different conditions. 
The bottom figures show the difference matrices when comparing the four test segments with one Forward-Day query segment. 
The stable data-association indicates the robustness of AutoMerge in multi-session revisits.

==> doc_review/exp/merge_pitt.tex <==
\subsection{Map Merging}
\label{sec:im_cluster}

So far, we have investigated the place recognition results between paired segments.
In this subsection, we consider the multi-segments offline/online map merging task on both the \textit{Pittsburgh} and \textit{Campus} datasets.

\subsubsection{Merging on \textit{Pittsburgh}}
\label{sec:pitt_merge}
In offline merging, we assume all the segments of interest have already been recorded, and AutoMerge can obtain the poses and features over all trajectories at test time.
Based on the relative connections among all the segments, AutoMerge can build the weighted graphs and cluster them into different sub-groups.
In Fig.~\ref{fig:off_pitts}, we evaluate the merging performance over different zones of the \textit{Pittsburgh} dataset.
We can notice that sub-maps in each zone have converged into one consistent large map.
However, not every segment has confident overlaps with other trajectories. 
Those segments with few interactions will be temporarily considered outliers.
For areas with multiple segment overlaps, AutoMerge can also detect the potential connections while ignoring relative viewpoint differences.
This property allows AutoMerge to have robust pose estimation with one-shot visits.
As shown in Table.~\ref{table:real_pr}, the merging performance is robust even in unknown environments.
When tested on the \textit{Pittsburgh} dataset, our model is trained on segments $1\sim10$ giving it $13\%$ dataset coverage. 
This training set only contains areas around Carnegie Mellon University.
The final merging results do not show a significant performance drop over the rest of the datasets, which contains varying terrain, open streets, and residential areas.
Because of its high generalization ability, AutoMerge does not require much data for training.

We also analyzed the robustness of offline clustering in the scenario where AutoMerge is given segments in a randomly selected order.
In Fig.~\ref{fig:merge_pitt_param}, we merged the segments for different values of parameter $C_{\omega}$.
For each parameter, we use a randomly generated $50$ segment streaming order, and calculate the corresponding clustering trends.
The results show that under all cases, AutoMerge can merge \textit{Pittsburgh} segments into $6$ major clusters, and the biggest cluster contains $43$ segments, as shown in Fig.~\ref{fig:off_pitts}.
From this, we can notice that the final clusters are not affected by the segment streaming order and the constant parameter $C_{\omega}$.


    
For incremental merging on the \textit{Pittsburgh} dataset, we assume all the segments are streamed incrementally.
In this case, at the early merging stage, we can only observe partial trajectories, and wrong matches are unavoidable with these short-term observations.
Using the incremental clustering method depicted in Sec.~\ref{sec:spectral}, AutoMerge can incrementally update the cluster property among segments.
Fig.~\ref{fig:online_merge_pitt} shows the incremental merging results over different maximum segment distances ($300m \sim 2400m$).
Fig.~\ref{fig:merge_pitt_distance} shows the total cluster size under different maximum segment distances.
In the $300m$ and $600m$ cases, the clusters have primarily merged into one cluster.
This is because AutoMerge cannot distinguish different sub-groups when all the connections are weak.
Beginning at the $900m$ distance, partial local overlaps are detected, and all $50$ segments are divided into $4\sim 6$ clusters during the merging procedure.
However, we can notice that not all cases can divided to $6$ clusters as we observed in the offline version of this task.
This is mainly caused by wrong connections between partial observations as indicated in Fig.~\ref{fig:online_merge_pitt}.
We highlight the wrong matches in red circles. These temporary outliers can break the global map as shown in the $1200m$ and $2100m$ cases.
But such failures can be quickly recovered from as shown in the green circles in the $1500m$ and $2400m$ cases. 
In the above experiments we also analyze how the streaming order affects merging for each maximum segment distance. 
The results show that AutoMerge's clustering ability is invariant to the streaming order.

==> doc_review/exp/pr.tex <==
    \begin{figure*}[t]
    	\centering
        	\includegraphics[width=0.9\linewidth]{Imgs/exp/pr/pr_curve_review.pdf}
        	\caption{\highlight{\textbf{Precision-recall Curves (PR-curve) on three datasets.}}
        	 On each dataset, the results are evaluated using testing and reference queries that have a relative translation of $2$m and relative rotation of $15^{\circ}$.
    	}
    	\label{fig:pr_curve}
    \end{figure*}

\section{Experimental Evaluation}
\label{sec:exp_eval}
As is shown in Table.~\ref{tab:dataset} and Fig.~\ref{fig:dataset}, AutoMerge can work with multiple overlaps under city-scale and campus-scale environments, and under various types of scenarios.
% Our place recognition results show that AutoMerge can handle variant viewpoint difference, where both traditional projection- or point- based approaches failed.
Overall, AutoMerge can achieve the best place recognition performance under varying viewpoint differences.
And the map merging results also indicate that data association and incremental merging of AutoMerge are not sensitive to parameter tuning and demonstrate higher generalization potential for new environments.
\replaced{Compared}{Comparing} with other learning-based methods, AutoMerge still shows robust data association ability on all the datasets, even though only trained on \textit{Pittsburgh} dataset.
% In general, because the we can notice that the competing methods suffer a performance drop when inferencing on the \textit{Campus} and \textit{KITTI} datasets, whereas
In this section, we will evaluate the place recognition accuracy, overlap retrieval accuracy, map merging efficiency, and computation efficiency respectively.

\subsection{Place Recognition Results}
\label{sec:PR_results}
\subsubsection{Orientation- and Translation- Tolerance Analysis}
\label{sec:ori_trans}

    We conduct experiments on three datasets to evaluate the robustness of place recognition of different methods. All learning-based methods are trained on tracks $1\sim 15$ of the Pittsburgh dataset.
    As shown in Fig.~9, we calculate the average Top-$1$ recall between query and reference frames(under translation differences $[1,2,3,4]m$ and yaw orientation differences $[15, 30]^{\circ}$).
    To generate orientation differences, we rotate each query frame by a desired angle and then apply a random noise uniformly sampled from the range $-2.5^{\circ}\sim 2.5^{\circ}$.
    The projection-based method, \deleted{M2DP and }SphereVLAD\cite{seqspherevlad}, can achieve orientation-invariance, but translation differences will greatly affect the recognition performance.
    Conversely, point-based methods can handle large translation differences but are sensitive to orientation differences.
    We can notice that AutoMerge has the translation-invariant property of point-based methods and orientation-invariant property of projection-based approaches. This is mainly due to our attention mechanism, which can reweigh the importance of the two branches in the feature extraction model.
    
    On both the \textit{KITTI} and \textit{Pittsburgh} datasets, AutoMerge outperforms both point-based and projection-based methods when subjected to large orientation and translation differences. 
    AutoMerge also shows great generalization compared to the single branch point-based and project-based approaches.
    \added{Moreover, the generalization ability of Automerge indicates the proposed attention fusion mechanism is not trained to overfit the training dataset.}
    \deleted{We can also notice that, the non-learning method M2DP also shows accurate place recognition, especially on \textit{KITTI} dataset.
    But the performance of M2DP will vary based on the 3D environments, which affects its map merging ability.}
    \added{We can also notice that MinkLoc3D shows consistent place recognition ability when dealing with significant translation noise.
    However, the same with other point-based methods, the performance declines with the increase of the viewpoint variance.}
    In Fig.~10, we analyze the PR-curve of different methods over three datasets.
    We can notice that both \deleted{SphereVLAD and }AutoMerge show\added{s} better performance than other descriptors\added{ in \textit{Pittsburgh} dataset}.
    On the other hand, since all the methods are only trained on \textit{Pittsburgh} dataset, there also exists general performance\deleted{s} drop for all the learning-based approaches over the rest two datasets.
    
    To investigate the merging ability, we analyze the merging accuracy over the \textit{Pittsburgh} and \textit{Campus} datasets.
    We extract \deleted{out }all the overlaps over the two datasets, and analyze the relative recalls and accuracy of the different methods.
    The results are shown in Table.\ref{table:real_pr}.
    \deleted{Non-learning method M2DP shows robust place recognition with high recall rates on one time visits. 
    With generated viewpoint differences, it cannot provide accurate data association for different time observations.
    This is mainly because the LiDAR mapping varies over the different revisits.
    Even though we utilize the dense mapping mechanism to enhance the local sub-maps' consistency, there may still exist dynamic mapping noise and mapping density differences.}
    \deleted{Compared to non-learning methods, all learning-based approaches show generalization on both datasets.}
    \deleted{And comparing with pure point- or projection- based approaches, AutoMerge shows higher precision and recall.}
    \added{As the distance of each submap is around 5$m$, the ability of the model to deal with variant orientation differences under translation differences around $2m \sim 3m$ is of vital importance.
    Automerge takes advantage of PointNetVLAD and SphereVLAD and achieves higher recall, compared with other methods.}
    This capability comes from the adaptive feature association, as stated in Section.~\ref{sec:fusion_network}.


==> doc_review/exp/setup.tex <==
\section{Datasets and Criteria}
\label{sec:data_crit}
    To evaluate the map merging accuracy, we choose the well-known \textit{KITTI}~\cite{DATASET:KITTI} dataset, one city-scale dataset collected in the City of Pittsburgh with around $\mathbf{120}$ km of trajectories in total, and one campus-scale dataset collected within Carnegie Mellon University with $\mathbf{4.5\times 8}$ km trajectories.
    The last two datasets are self-recorded with our data-collection platform, and they contain multiple revisits, as well as translation and orientation differences.
    In this section, we describe the datasets, target methods, and evaluation criteria.
    
    \bigskip
    \noindent \textbf{Merging Datasets:} To cover various scenarios in our datasets, we travel through different types of areas over our self-gathered datasets, and we include multiple revisits.
    The  detailed characteristics of each dataset and the environment will be provided in the following descriptions. 
    Fig.~\ref{fig:dataset} shows the overlaid segments on an aerial map, which illustrates the segment shapes, scales, and areas. The details are summarized in Table~\ref{tab:dataset}.
    
   \begin{table} [htbp]
        \caption{Comparison of different map merging approaches.}
        \centering
        \begin{tabular}{|C{1.5cm}|C{4cm}|C{1.5cm}|}
            \hline
            \textbf{Dataset}
            & \textbf{Environments}
            & \textbf{Scales (km)}
            \\
            \hline
            KITTI~\cite{DATASET:KITTI} & Street & $15\times 1$\\
            \hline
            Pittsburgh & Street, Residential, Terrain & $120\times 1$\\
            \hline
            Campus & Campus area & $4.5\times 8$\\
            \hline
        \end{tabular}
        \label{tab:dataset}
    \end{table}
    
    
    \begin{itemize}
        \item \textbf{Pittsburgh} dataset is collected within the city of Pittsburgh with our data-collection platform, which contains a Velodyne-16 LiDAR scanner, Xsens MTI-300 inertial measurement units, and GNSS position systems.
        The collected areas (open street, residential areas, commercial buildings, etc.) contain $50$ trajectories with a total distance of $120$ km and $158$ overlaps.
        \item \textbf{Campus} dataset is recorded with the same data-collection platform within the campus area of Carnegie Mellon University (CMU).
        The collected data covers $10$ main trajectories throughout the campus, where each trajectory is recorded $8$ times under different conditions (illuminations, directions, etc).
        The total length is around $36$km.
        \item \textbf{KITTI} dataset is a well-known dataset for autonomous driving in urban environments.
        We extract out $10$ (around $15$km in total) trajectories from \textit{KITTI} odometry dataset, and mainly used it to evaluate the generalization ability of our place recognition.
    \end{itemize}
    
    Due to sparse LiDAR scanning, occlusion, and changes in perspective, the same place may be represented by different observations.
    To provide consistent local maps for feature extraction, AutoMerge generates a dense map with traditional LiDAR odometry~\cite{LOAM:zhang2014loam}. This approach has been applied in our previous work~\cite{fusionvlad}.
    For each place, sub-maps are constructed by accumulating LiDAR scans into dense observations and keeping a distance ($40$m) to the vehicle's latest position.
    The sites in the CMU campus and \textit{KITTI} datasets have a maximum of two lanes and large lateral displacement with no exceptions.
    The sites in the Pittsburgh dataset street areas have two to four lanes, which indicates a certain lateral displacement during inverse observation.
    The major differences between the \textit{Campus} dataset and the other datasets is the multiple re-visits over the same segments.
    We extract sub-maps every $5$m with a fixed $50$m radius. Fig.~\ref{fig:dense_map} shows example extracted sub-maps.
    These maps can only be extracted when the relative distance between the vehicle's central point and the keyframe's is $100$m away.
    In this manner, the geometric structures for the same areas will be very similar in both under forward and reverse traversal directions. 
    The above datasets enable us to evaluate  place recognition accuracy against rotational and lateral changes, refine data-association robustness against outlier wrong matches, and test map merging performance under large-scale environments.
    In all of the above datasets, we count the retrieval as successful if the detected candidates are $10$m apart from the ground-truth positions.

    \bigskip
    \noindent \textbf{Evaluation Criteria:} To evaluate the loop closure detection accuracy and map merging performance, we use the following three metrics:
    
    1) \textit{Recalls@Top$N$ Retrievals}: AutoMerge uses the best retrievals for map merging, and accurate place retrieval should be invariant to perspective differences.
    We utilize Top-$1$ recall as the main evaluation metric to analyze the place recognition robustness under changing viewpoints.
    
    2) \textit{Precision-Recall Curve}: recall cannot fully represent the general place recognition ability for global merging, as high false positives will make the map optimization fragile even with high recall.
    To this end, we utilize the precision-recall between different segments to investigate the accuracy of retrievals, and the generalization ability for unknown datasets.
    
    3) \textit{Merging Accuracy}: the above metrics mainly focus on fine-grained place recognition accuracy, and cannot fully encapsulate the performance in map-merging tasks.
    Since localization accuracy analysis (i.e., Mean Squared Error) is not realistic for large-scale merging, especially when odometry drift will be a part of the error, AutoMerge use a simplified merging metric.
    We notice that even limited accurate retrievals ($2\sim 4$) on overlaps can provide accurate map merging results.
    For coarse-grained place retrieval accuracy, we care more about the overlaps' binary retrieval rates, i.e., $0/1$ for found/missed.
    
    \bigskip
    \noindent \textbf{Targeting Methods:}
    To analyze the place retrieval accuracy, we compare the fusion-enhanced descriptor extraction of AutoMerge with other state-of-the-art 3D place recognition \added{learning-based }methods:
    \deleted{1) M2DP~\cite{Feature3D:M2DP} for non-learning based methods, and 2) }PointNetVLAD~\cite{PR:pointnetvlad}, PCAN~\cite{PR:pcan}, LPD-Net~\cite{liu2019lpd}, \added{SOE-Net~\cite{PR:soe}, MinkLoc3D~\cite{LPR:minkloc3d} and} SphereVLAD~\cite{seqspherevlad} \deleted{for learning-based method}.
    In all the above methods, we use the same sub-map configuration, i.e. $5m$ distance between keyframes, and $50m$ radius and $0.5m^3$ voxelization for each sub-map as shown in Fig.~\ref{fig:dense_map}.
    For map merging evaluation, we only use Top-1 retrieval to detect overlaps among segments, and apply \textit{Merging Accuracy} to provide quantitative analysis and relative quality demonstration to investigate the merging details.
    Please note that point-based methods usually cannot find overlaps in the reverse traversal direction ($180^{\circ}$).
    For a fair comparison, we store the local features for both forward and reverse directions.
    Given the testing and reference queries, we calculate both distances ($cos(f_{ref}^{forward},f_{test}^{forward})$ and $cos(f_{ref}^{forward}, f_{test}^{reverse})$), and use the minimum as the place feature distance.

    \begin{figure*}[t]
        \centering
        \includegraphics[width=0.9\linewidth]{Imgs/exp/pr/recall_review.pdf}
        \caption{\highlight{\textbf{Localization results for different viewpoints on different datasets.}}
        For each dataset, we pick one segment from the same domain and generate test/reference queries with different yaw angles $[15,30]^{\circ}$ and translational displacement $[1,2,3,4]m$, and then analyze the average recall for top-$20$ retrievals.
        }
        \label{fig:recall_analysis}
    \end{figure*}

To evaluate the generalization of the place recognition and data-association, we used only \textbf{30\%} of the \textit{Pittsburgh} dataset (which is \textbf{20\%} of the total of all three datasets) to train different learning-based methods, and inference over the remaining datasets with the trained models.

==> doc_review/intro.tex <==
\section{Introduction}
\label{sec:introduction}

    \begin{figure}[t]
        \begin{center}
          \includegraphics[width=\linewidth]{Imgs/intro/idea.pdf}
        \end{center}
        \caption{\textbf{Map Merging in the City of Pittsburgh.}
        Map merging for $50$ segments in the City of Pittsburgh, Pennsylvania, USA.
        The mapped areas include Shadyside, Squirrel Hill, Bloomfield, etc, totaling $180km$ in distance.
        AutoMerge can detect their inner connections without initial estimation, and achieve global mapping through rough/refined merging procedures.
        }
        \label{fig:idea}
    \end{figure}

    \IEEEPARstart{L}{arge}-scale 3D mapping is one of the fundamental topics in robotics research due to its capacity to provide accurate localization and 3D environment representation for high-level perception and planning tasks.
    % no overlaps, server-abased assembling, 
    % Segments, need define
    % Accurate map merging in large-scale environments is heavily relied on for various applications, such as (i) autonomous driving and last-mile delivery, where one single agent may re-visit the same trajectory multiple times, and (ii) multi-agent exploration in search-and-rescue tasks and surveillance, allowing different agents to start from their own coordinates.
    For both single- and multi-agent mapping systems, merging coupled segments into the same world coordinates becomes necessary to generate accurate localization and mapping results.
    However, as shown in Fig.~\ref{fig:idea}, accurate map merging without initial \added{coordinate }estimation\added{ (i.e., the relative transformations between agents)} in large-scale environments is still an unsolved problem, since \added{the }relative transformation between segments \replaced{is}{are} unknown.
    Factors that contribute to the difficulty of this problem include:
    % The wrong matches are mainly caused by two factors:
    \begin{itemize}
        \item Loop closures are susceptible to both translation and orientation differences; when re-visiting the same area, the place descriptor will vary under different perspectives.
        \item Different areas may share similar geometries, such as a long street, a highway, etc., which may cause incorrect data associations among segments without overlaps.
        \item Most methods are extremely sensitive to failed matches; even a few incorrect data associations between segments can turn the global map optimization into an ill-posed problem. 
    \end{itemize}
    
    \noindent Traditional map merging approaches rely on good initialization~\cite{Merge:LAMP} and accurate odometry estimation.
    For a single agent revisiting an area or a multi-agent system without prior knowledge, previous works utilize RANSAC~\cite{lpr:ransac} to filter out incorrect matches via Euclidean constraints.
    However, such methods are highly reliant on the discriminability of unique areas, which is hard to guarantee in both \deleted{of the }scenarios mentioned above. 
    
    % Insight for place descriptor
    In this work, we propose a 3D mapping system, AutoMerge, that enables \replaced{robust}{real-time} and accurate large-scale map merging under significant viewpoint differences.
    % without any initial relative location estimates between trajectories.
    \replaced{Without any initial estimation, AutoMerge can provide reliable loop closures for an initial rough alignment between different trajectories and then perform global reformation for all the incoming trajectories.}{without any initial relative location estimates between trajectories}
    For either single-agent segment revisiting or multi-agent collaboration mapping, perspective differences and incomplete observations can occur in the 3D representations for the same area, and traditional descriptors~\cite{PR:pointnetvlad, PR:overlapnet} are sensitive to the above scenarios.
    In general, a point-/voxel-based feature extraction approach is designed to be translation-invariant; however, the local viewpoint differences (especially in a detour) can affect the extracted local features.
    In our previous work, we notice that spherical projection shows advanced performance under orientation differences~\cite{spherevlad}, and multi-perspective fusion\cite{fusionvlad} can provide robustness against viewpoint differences.
    In AutoMerge, we develop a novel multi-perspective fusion-based approach for a 3D place descriptor, which combines different perspective-invariant properties \cite{fusionvlad, spherevlad} by leveraging the network features with additional attention-based~\cite{attention_all_your_need} fusion layers.
    As a result of the new place descriptor, AutoMerge can provide the highest average recall rates and lowest false positive rates compared to other state-of-the-art methods.
    Our descriptor can be extracted in real-time, making it suitable for both accurate offline merging for map refinement, and fast incremental\deleted{-online} merging for multi-agent mapping.


    % Insight for data association
    Perceptual aliasing caused by similar scenarios (long streets, crossroads\replaced{,}{ and} highways, etc.) often results in incorrect data association.
    Such failures can cause catastrophic problems in\deleted{ the} back-end optimization.
    Most traditional place retrieval methods are based on single scan estimation~\cite{VPR:DBOW2}\added{,} which heavily relies on good initial coordinates, or brute-force sequence searching~\cite{MRS_VPR}, which works only for large overlaps.
    This work addresses this challenge by developing a hybrid loop closure estimation module.
    We notice that: 1) sequence matching \cite{2012SeqSLAM} can provide high recall and accuracy over long consistent overlaps but not in areas with few scan overlaps; 2) RANSAC-based single scan matching \cite{1981RANSAC, 2015Robust} can handle areas with short overlaps but may introduce inter-outliers\added{ (i.e., wrong matching between overlapped trajectories)} for long-distance segments with similar geometry patterns.
    To detect matches with high accuracy, we formulate an adaptive loop closure detection mechanism by balancing the place retrieval mechanisms mentioned above.

    \bigskip
    \textbf{The contributions} of AutoMerge can be summarized as:
    \begin{itemize}
        \item AutoMerge provides a framework that can merge segments in city-scale environments without requiring initial\added{ coordinates} estimations.
        Using this framework, we enable multi-agent map merging by being invariant to relative perspective differences and temporal differences.
        \item Within AutoMerge, we design an adaptive loop-closure detection module, which provides high recall and low false positive place retrievals, resulting in significantly reduced outliers in repeated environments during large-scale merging.
        \item AutoMerge \replaced{can}{has the ability to} perform incremental map merging for single- and multi-agent systems. This procedure is invariant to the data streaming order from the different agents \deleted{both} in the temporal and spatial domain and to the revisit times for the same area.
        \item Extensive evaluation on different large-scale datasets.
        We demonstrate detailed qualitative and quantitative analysis on the public \textit{KITTI}~\cite{DATASET:KITTI} dataset and on our \deleted{own }city-scale and campus-scale datasets, which show that AutoMerge provides accurate map merging performance, and also that it has high generalization for unknown areas.
    \end{itemize}

    \bigskip
    \textbf{Novelty with respect to previous work~\cite{spherevlad,fusionvlad,adafusion}:}
    Our previous works investigate orientation-invariant~\cite{spherevlad} and translation-invariant~\cite{fusionvlad} 3D Loop Closure Detection (LCD). 
    Firstly, with a better understanding of features' robustness under different perspectives and our previous robust fusion-based data-association~\cite{adafusion}, AutoMerge presents an attention-enhanced multi-view fusion descriptor to improve the robustness under both translation and orientation differences simultaneously.
    Secondly, AutoMerge has an adaptive loop closure detection mechanism to maintain highly accurate loop closure detection with high recall rates.
    The above advantages allow AutoMerge to provide an offline map merging system for previously-stored 3D sub-maps, and an incremental map merging framework for single- and multi-agent mapping\added{, which can further benefit the crowd-sourced mapping in current last-mile delivery and autonomous driving}.


==> doc_review/method/feature.tex <==
\begin{figure*}[t]
    \centering
        \includegraphics[width=\linewidth]{Imgs/method/Net_review.pdf}
        \caption{\highlight{\textbf{The network structure of the AutoMerge descriptor extraction.}}
        To provide viewpoint-invariant descriptor extraction, our network includes a point-based branch to improve the robustness \replaced{of}{to} translation differences\deleted{,} and a sphere-based branch for rotation differences.
        Finally, AutoMerge utilizes a deep fusion mechanism between the two branches, which can enhance the individual branches and the joint branch simultaneously.
        }
    \label{fig:flowchart}
\end{figure*}

\section{Fusion-enhanced Descriptor Extraction}
\label{sec:fuse_dis}
    As analyzed in Sec.~\ref{sec:related_works}, point-based approaches show better performance against translation differences when compared with projection-based methods, whereas projection-based methods show better accuracy against orientation differences.
    Our fusion-enhanced descriptor balances the advantages of both point- and projection-based approaches with a multi-perspective feature extraction network.
    As shown in Fig.~\ref{fig:flowchart}, the network includes two core components: 1) a multi-perspective feature extraction module, 
    and 2) an attention place feature fusion module.
    
\subsection{Multi-perspectives Feature Extraction}
    \label{sec:MFE}
    Due to the sparsity and occlusion problems of a raw LiDAR scan, a 3D observation will vary when gathered under different viewpoints.
    To provide stable multi-perspective feature extraction, we first accumulate the point cloud into local dense maps.
    This mechanism can provide a consistent local dense map based on LiDAR odometry estimation, which has been explained in detail in our previous work~\cite{fusionvlad}.
    In the following subsections, we provide details on how we utilize point-based and projection-based feature extraction in our method.
    
    \bigskip
    \noindent \textbf{Point-based Feature Extraction:}
    \label{sec:point-view}
    In this branch, we adopt the idea of PointNetVLAD\cite{PR:pointnetvlad} to extract the global descriptor. 
    % To alleviate the sensitivity in rotation differences, we design a rotation-enhanced mechanism by encoding the point cloud in two opposite directions.
    % Given point cloud $P=\{p_1,...p_N|p_n \in \mathbb{R}^3\}$, the corresponding rotated point cloud $P_{rot}$ is derived from $P_{rot}=R_{180}P$, where $R_{180}$ is the rotation matrix along $Z$-axis by $\pi$.
    % Then, both $P$ and $P_{rot}$ are fed into a shared-weight PointNet\cite{feature:pointnet} to obtain local features $F_p=\{f_1,...f_N|f_n \in \mathbb{R}^C\}$ and $F_{p\_rot}=\{f_1^\prime,...f_N^\prime|f_n^\prime \in \mathbb{R}^{C_p}\}$, which results in fused local features $F_{p\_fused} \in \mathbb{R}^{2N \times C_p}$ by concatenating them together.
    % To improve place retrieval ability with rotation uncertainty of point cloud, we utilize NetVLAD~\cite{NetVLAD} layer to learn and cluster feature centroids for both original and rotated features to generate equivalent global descriptors $V_{point} \in \mathbb{R}^{(N_c\times C_p)}$ for both direction, where $N_c$ is the cluster number of NetVLAD layer.
    % Finally, global descriptor $V_{point}$ is applied with a fully connected layer to yield a compact descriptor.
    Given a local dense map, we query the points set $P=\{p_1,...p_N|p_n \in \mathbb{R}^3\}$ within a $80m \times 80m$ bounding box and preprocess it as shown in \cite{PR:pointnetvlad}. 
    Then, $P$ is fed into PointNet\cite{feature:pointnet} to extract local features $F_p=\{f_1,...f_N|f_n \in \mathbb{R}^C_{p}\}$.
    With the help of a NetVLAD layer\cite{NetVLAD}, the global descriptor $V_{point}$ is obtained by aggregating local point features. 
    Finally, the global descriptor $V_{point}$ is run through  a fully connected layer to yield a compact descriptor.
    

    
    \bigskip
    \noindent \textbf{Projection-based Feature Extraction:}
    \label{sec:sph-view}
    % \cite{sh}
    To obtain viewpoint invariance, we utilize the spherical convolution\cite{cohen2018spherical} to extract local features from a spherical projection of the point cloud. 
    Using the local dense maps, we query the points within a range of $50m$ and project them into a panorama using the method mentioned in \cite{fusionvlad}. 
    Then the corresponding spherical projection $SP \in \mathbb{R}^{H \times W}$ is fed into 4 layers of spherical convolutions to generate local features $F_s \in \mathbb{R}^{C_s \times \alpha \times \beta \times \gamma}$ which contain features sampled from angles in all three axes.
    A NetVLAD~\cite{NetVLAD} layer is used to find the spatial similarities between local features and reorder them in a specific manner.
    Finally, the global descriptor $V_{sphere}$ is also run through a fully connected layer to reduce the feature dimensions.

    \begin{figure}[t]
    	\centering
        	\includegraphics[width=\linewidth]{Imgs/method/Fusion.pdf}
    	\caption{\textbf{Attention-enhanced Feature Extraction.}
    	For each branch, AutoMerge applies a self-attention layer to improve the network feature extraction.
    	Between the two branches, AutoMerge also applies a cross-attention layer to enhance their inner connections.
    	}
    	\label{fig:fusion_layer}
    \end{figure}

\subsection{Attention Fusion}
\label{sec:fusion_network}
Our attention fusion module consists of two self-attention modules providing contextual information for $V_{point}$ and $V_{sphere}$ individually, and a cross attention module which aims to reweigh the importance of channels within the concatenation of $V_{point}$ and $V_{sphere}$.

    \bigskip
    \noindent \textbf{Self-attention Feature Enhancement:}
    Each channel of the global descriptor can be interpreted as a specific response and different combinations of channels can be regarded as different patterns of the environment \cite{att:dual_attention}. 
    However, when extracting the local features, PointNet\cite{feature:pointnet} only considers each point independently and the receptive field of the spherical convolution is also limited by the number of layers, which leads to a lack of inter-channel dependencies in global descriptors.
    By exploring the inter-dependencies between channels, we can therefore enhance the semantic information representation of the global descriptor.
    \begin{align}
        V_{SA} &= V + \gamma \text{SoftMax}(V V^{T})^{T}V
    \end{align}
   
       \begin{figure*}[ht]
    	\centering
        	\includegraphics[width=\linewidth]{Imgs/method/lcd.pdf}
    	\caption{\textbf{Illustration of Adaptive Loop Closure Detection.}
    	(i) The figure shows the difference matrix between two segments, where the red points indicate the potential matches via sequence matching~\cite{2012SeqSLAM}\deleted{ shown in yellow}. 
    	(ii) The matches are clustered into individual zones via K-means based on their feature distances.
    	(iii) RANSAC is utilized to exclude outliers that can not satisfy Euclidean constraints.
    	}
    	\label{fig:adaptive_lcd}
    \end{figure*}
    
    Given a global descriptor $V \in \mathbb{R}^{C \times 1}$, we obtained the attention map $A \in \mathbb{R}^{C \times C}$ by directly multiplying $V$ and its transpose and applying a SoftMax function on the result along the row direction.
    Each element $A_{ji}$ represents the impact of $j^{th}$ channel on $i^{th}$ channel.
    Then, we multiply the transpose of attention map $A$ with $V$ to generate a weighted sum of every channel which contains the inter-channel dependencies.
    Finally, we multiply the result with a learnable parameter $\gamma$ to scale the inter-channel dependencies and add it with $V$.
    

    
    \bigskip
    \noindent \textbf{Cross-attention Feature Reweighing:}
    While inter-channel dependencies can provide contextual information, they can also evaluate the contribution of each channel.
    During feature fusion, there are situations that are only beneficial to one of the branches, and so simple concatenation of the two global descriptors will lead to a large performance decrease.
    Inspired by~\cite{att:channel_attention}, our cross-attention feature reweighing module learns the inter-channel dependencies and emphasizes the more meaningful channels and neglects the irrelevant channels.
    
    The network structure is illustrated in Fig.\ref{fig:fusion_layer}. The input is concatenation of two global descriptor $[V_{point}, V_{sphere}]$ denoted as $V_{cat} \in\mathbb{R}^{2C \times 1}$.
    We directly get the correlation matrix $E$ from multiplication of $V_{cat}$ and its transpose.
    \begin{align}
        E = V_{cat} V_{cat}^{T}
    \end{align}
    Then, we average the elements in each row of the $E$ to aggregate the responses of each channel, and multiply $E$ with the result to obtain channel correlation weight $\alpha_{corr}$.
    We further utilize a fully connected layer to exploit the dependencies of channels and apply a Sigmoid function to narrow the channel importance weight $\alpha_{w}$ within $[0,1]$.
    \begin{align}
        \alpha_{corr} = E\otimes \text{Ave\_Pool}(E) \\
        \alpha_{w} = \text{Sigmoid}(W(\alpha_{corr}))
    \end{align}
    Finally, we apply an element-wise multiplication between channel importance weight $\alpha_{w}$ and $V_{cat}$ to yield the attention-reweighted global descriptor.
    \begin{align}
        V_{CA} = \alpha_{w} \odot V_{cat}
    \end{align}

\subsection{Learning Metrics}
\label{sec:loss}
To enable end-to-end training for our network, we utilize the "Lazy quadruplet" loss metric.
Sets of training tuples are selected from the training dataset and each of these training tuples is composed of four components: $\mathcal{S} = [S_a, \{S_{pos}\}, \{S_{neg}\}, S_{neg^{*}}]$, where the $S_a$ represents the query frame location at the ground truth position, $\{S_{pos}\}$ stands for a set of ``positive" frames whose distance to $S_a$ is less than the threshold $D_{pos}$, $\{S_{neg}\}$ denotes a set of ``negative" frames whose distance to $S_a$ is strictly larger than threshold $D_{neg}$ and $S_{neg^{*}}$ represents a frame whose distance to $\{S_{neg}\}$ is strictly larger than $D_{neg}$.
In our case, these two thresholds are set as $D_{pos}=10m$ and $D_{neg}=50m$.
The lazy quadruplet loss is defined as
\begin{align}
    L_{lazyQuad}(\mathcal{S}) = &\max_{i, j}([\gamma + \delta_{pos_i} - \delta_{neg_j}]_{+})  +  \\ &\max_{i,k}([\alpha + \delta_{pos_i} - \delta_{neg_k^{*}}]_{+}) \nonumber
\end{align}
where $\alpha$ and $\beta$ are the constant threshold giving the margin and $[...]_{+}$ denotes the hinge loss. 
% In our case, $\alpha$ and $\beta$ are set to $1.0$ and $0.5$.

==> doc_review/method/lcd.tex <==
\section{Adaptive Loop Closure Detection}
\label{sec:lcd}
    In our AutoMerge framework, loop closures are required to be accurate (few false positives) and robust (high recall), though these two properties are contradictory.
    As shown in Fig.~\ref{fig:adaptive_lcd}, our adaptive loop closure detection module can estimate the stable data-association while ignoring the potential outliers, through our sequence matching and RANSAC filtering mechanisms.
    In this section, we will introduce details.

\subsection{Adaptive Candidates Association}
    In order to find possible loops among multiple segments, they are grouped into pairs for every two segments $T_i$ and $T_j$ $(i \ne j)$. Each $T_i$ has point cloud sub-maps separated by a constant distance and the corresponding poses $\mathbf{T}_i = \{\mathbf{T}_i^k\}$, both of which are obtained from the odometry. These sub-maps are then encoded with our fusion-enhanced descriptor and represented as feature $\boldsymbol{f}_i = \{\boldsymbol{f}_i^k\}$. 
    The similarity of places (i.e. sub-maps) of different segments can be revealed in the difference matrix $\mathbf{D} = \mathrm{d}(\boldsymbol{f}_i, \boldsymbol{f}_j) \in \mathbb{R}^{N_i \times N_j}$, where $\mathrm{d}(\cdot)$ is the cosine distance and $N_i$ and $N_j$ are the number of sub-maps in $T_i$ and $T_j$ respectively.
    
    Our adaptive LCD method works on loop candidates $\mathcal{C} = \{(k_i, k_j)\}$ where $k_i$ and $k_j$ are the index of submaps in $T_i$ and $T_j$, showing the association of places in a segment pair.
    We acquire $\mathcal{C}_\mathrm{seq}$ by applying sequence matching \cite{2012SeqSLAM} on the difference matrix $\mathbf{D}$.
    However, as we can see in Fig.~\ref{fig:adaptive_lcd}, the raw match result still exists lots outliers.
    To filter them out, we utilize kmeans to cluster the potential matches into different zones ${\mathcal{C}_\mathrm{seq}}_i,i=1,...,k$ via k-means based on the feature distances.
    Then for $i$-th zone, we adopt the idea of RANSAC to select correspondences from ${\mathcal{C}_\mathrm{seq}}_i$, with an edge-based geometric consistency principle to check the correctness of the proposal of correspondences.
    Specifically, within each iteration, the relation
    \begin{equation}
        \|\mathrm{edge}_i \|_2 \ge \beta \|\mathrm{edge}_j \|_2, \qquad
        \|\mathrm{edge}_j \|_2 \ge \beta \|\mathrm{edge}_i \|_2
    \end{equation}
    is checked between $n$ samples $(k_i, k_j)$, where the edges are formed by every two samples $(k_i^1, k_j^1)$ and $(k_i^2, k_j^2)$, and $\beta \in [0, 1]$ controls the degree on equality of edge length.
    Through the above mechanism, AutoMerge can filter out most outliers.
    
    % To prepare robust $\mathcal{C}_\mathrm{ran}$ for the RANSAC-based single scan matching, a strict bidirectional nearest neighbor strategy is used, which satisfies
    % \begin{equation}
    %     k_i = \arg \min{\mathbf{D}_{:,k_j}}, \qquad
    %     k_j = \arg \min{\mathbf{D}_{k_i,:}},
    % \end{equation}
    % where $\mathbf{D}_{k_i,:}$ is the $k_i$-th row of $\mathbf{D}$ and $\mathbf{D}_{:,k_j}$ is the $k_j$-th column of $\mathbf{D}$.

\color{red}
% \begin{algorithm}[t]
% \caption{Adaptive Loop Closure Detection}
% \label{alg:adaptive_lcd}
% \begin{algorithmic}[1]
%     \renewcommand{\algorithmicrequire}{\textbf{Input:}}
%     \renewcommand{\algorithmicensure}{\textbf{Output:}}
%     \Require Loop candidates $\mathcal{C}_\mathrm{seq}$ and $\mathcal{C}_\mathrm{ran}$
%     \Ensure Correspondences $\mathcal{C}_\mathrm{gt}$
%     \State $\mathcal{C}_\mathrm{seq}^\prime \gets $ \Call{SeqFiltering}{$\mathcal{C}_\mathrm{seq}$}
%     \If{$|\mathcal{C}_\mathrm{seq}^\prime| \ne 0$}
%         \State $\mathcal{C}_\mathrm{gt} \gets $ \Call{RansacFiltering}{$\mathcal{C}_\mathrm{seq}^\prime$}
%     \Else
%         \State $\mathcal{C}_\mathrm{gt} \gets $ \Call{RansacFiltering}{$\mathcal{C}_\mathrm{ran}$}
%     \EndIf
%     \State \Return{$\mathcal{C}_\mathrm{gt}$}
% \end{algorithmic}
% \end{algorithm}

% \subsection{Adaptive Data Association}
%     The distribution of outliers in $\mathcal{C}_\mathrm{seq}$ and $\mathcal{C}_\mathrm{ran}$ share a different pattern.
%     Loop candidates from sequence matching appear similar to many segments since it focuses on local continuity. 
%     We can then use parameters such as segment length and slope to filter out noise and select the best segments as correspondences.
%     However, candidates from $\mathcal{C}_\mathrm{ran}$ are usually sparse and not close to each other because they are the global minimums in $\mathbf{D}$ for sub-map matching.
%     We adopt the idea of RANSAC to select correspondences from $\mathcal{C}_\mathrm{ran}$, with an edge-based geometric consistency principle to check the correctness of the proposal of correspondences.
%     Specifically, within each iteration, the relation
%     \begin{equation}
%         \|\mathrm{edge}_i \|_2 \ge \beta \|\mathrm{edge}_j \|_2, \qquad
%         \|\mathrm{edge}_j \|_2 \ge \beta \|\mathrm{edge}_i \|_2
%     \end{equation}
%     is checked between $n$ samples $(k_i, k_j)$, where the edges are formed by every two samples $(k_i^1, k_j^1)$ and $(k_i^2, k_j^2)$, and $\beta \in [0, 1]$ controls the degree on equality of edge length.
%     With the above sequence filtering and RANSAC filtering methods, we generate true correspondences $\mathcal{C}_\mathrm{gt}$ in an adaptive cross validation manner, as stated in Algorithm~\ref{alg:adaptive_lcd}.

\color{black}


==> doc_review/method/ml.tex <==
\section{Incremental Merging}
\label{sec:inc_merge}
For the large-scale merging task, we may encounter \replaced{a}{the} case where there exist\deleted{s} more than two groups of segments with overlaps.
The overlaps between segments are limited at the early stage and can be extended at the late stage.
In \deleted{the }merging\deleted{ procedure}, \replaced{the manner used to divide}{dividing} all segments into\deleted{ different} groups with stable connections is essential for incremental factor graph optimization.
\replaced{In this section, we}{This section will} introduce the details of our incremental merging mechanism.

\subsection{Multi-agent Clustering}
\label{sec:spectral}

Firstly, we formulate the incremental merging task into a traditional spectral clustering problem~\cite{spectral_cluster}.
Assume there exists $V=\{v_1, ..., v_n\}$ agents running \replaced{independently}{in the real time}, and we \replaced{define}{can evaluate} the replaced{inner connection $\omega_{ij}\sim [0,1]$}{inner connections} between $v_i$ and $v_j$\replaced{, which indicates the overlap confidence of agent $v_i$ and $v_j$ existing stable overlaps}{ as $\omega_{ij}$}.
Without losing generality, we define a weighted graph $G=(V,E)$. $E$ represents the edge connections, which satisfies $\omega_{ij}=\omega_{ji}$.
We define $A_i,i=1,...k$ as the subset of $V$, and satisfies $A_1 \cup ... \cup A_k = V, A_i\cap A_j=\emptyset$, $\bar{A_i}$ is the complement of $A_i$.
And $W(A_i, \bar{A_i})$ is weighted adjacency matrix, which is defined as,
\begin{align}
    W(A_i, \bar{A_i}) := \sum_{k \in A_i, l \in \bar{A_i}} \omega_{kl}
    \label{eq:adjacency}
\end{align}

\begin{figure}[t]
	\centering
    	\includegraphics[width=\linewidth]{Imgs/method/cluster.pdf}
	\caption{\textbf{Incremental Merging.}
	(1) Graph $G=(V,E)$ is constructed with $V=\{v_1,...,v_n\}$ agents and their connections $\omega_{ij}\in E, i\neq j$.
	(2) AutoMerge can incrementally merge agents into different sub-groups by maximizing the inner connections within each sub-group and minimizing the connections between sub-groups.
	(3) When a new node $v_{11}$ builds new confident connections with $v_5$ and $v_8$, or previous connection $\omega_{2,8}$ is re-enhanced, AutoMerge can update the sub-groups into a joint group.
	}
	\label{fig:inc_merge}
\end{figure}

From the loop closure detection perspective, the inner connection $\omega_{ij}$ between agent $v_i$ and $v_j$ is based on overlap length and place recognition quality.
Thus, we define inner connection $\omega_{ij}$ as,
\begin{align}
    \omega_{ij} = \left\{ 
    \begin{array}{cc}
         &  \exp \left(-\frac{\|F_i - F_j\|_2^2+C_{\omega}}{2L_{ij}^2+\epsilon} \right), i\neq j \\
         & 0, i=j
    \end{array}
    \right.
    \label{eq:connection}
\end{align}
where $F_i$ indicates the extracted overlap place features from agent $v_i$, and $L_{ij}$ is the length of overlap area.
$C_{\omega}$ is a hyper-parameter to control the $\omega_{ij}$'s dependence on the overlaps' length, and $\epsilon=1e-4$ is a constant parameter.
In the extreme cases where $\|F_i - F_j\|_2^2 \ll C_{\omega}$, the weighting $\omega_{ij}\sim \exp \left(-\frac{C_{\omega}}{2L_{ij}^2} \right)$ will mainly depend on the length of overlaps.
Based on \added{the }above equation, we can also define degree matrix $D$, where $d_{ii}=\sum_{j=1}^n \omega_{ij}$ and is the connection measurement between agent $v_i$ with all other agents $\bar{v_i}$.
According to spectral clustering~\cite{spectral_cluster}, the incremental merging task can be defined as a mincut problem, 
\begin{align}
    \min cut(A_1,...,A_k) := \min \frac{1}{2}\sum_{i=1}^k W(A_i, \bar{A_i})
\end{align}
The major limitation of the above mincut is that it will simply separate one individual agent $v_i$ from the rest of agents $\bar{v_i}$, which is not our desired map segmentation. 
To maintain sub-groups with a large size, we utilize the object function from Ncut~\cite{ncut},
\begin{align}
    \min Ncut(A_1,...,A_k) &:= \min \frac{1}{2}\sum_{i=1}^k \frac{W(A_i, \bar{A_i})}{vol(A_i)} \\
    vol(A_i) &:= \sum_{j\in A_i} d_{jj}
\end{align}
where $vol(A_i)$ is the measurement of inner connections among the sub-group $A_i$.
From the power consumption perspective, incremental clustering is trying to find the best segment option with \added{a }minimum penalty to divide the original agents into different consistent sub-groups.

The solution to the Ncut problem is detailed in the reference~\cite{spectral_cluster}, and the standard spectral cluster approach \replaced{is}{as} shown in Algorithm~\ref{alg:spectral}. 
Given the agent list $V=\{v_1,...,v_n\}$, we can calculate the similarity matrix (Eq.~\ref{eq:connection}), degree matrix $D$, and corresponding Laplace matrix $L$.
The eigenvalues $\lambda_k, k=1,...,n$ can indicate the clustering status.
In theory~\cite{spectral_cluster}, if there exist $k$ different sub-groups $\{A_1,...,A_k\}$ without connections $W(A_i, A_j)=0, i\neq j$, the number of eigenvalues $\lambda_i = 0$ equals to $k$.
In the map merging problem, partial overlaps between different sub-groups may exist, thus we set a control threshold ($\lambda_{max} \leq \theta$) to estimate the best sub-groups size.
Based on the first $k$-dimension of eigenvectors $\mathcal{U}$, we can construct a key matrix $\mathcal{K}^{n\times k}$, and cluster to $k$ classes though $k$-means.
Through the above operation, AutoMerge can cluster agents into $k$ sub-groups.

\begin{algorithm}[t]
\caption{Incremental Clustering}
\label{alg:spectral}
\begin{algorithmic}[2]
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \Require Agent list $V=\{v_1,...,v_n\}$
    \Ensure Clusters $A_1,..., A_k$ with $A_i \in \{j|y_j \in \mathcal{R}^k\}$
    \State Construct similarity graph $W$, and $\omega_{ij}$ based Eq.~\ref{eq:connection} 
    \State Construct degree matrix $D$, and $d_{ii}=\sum_{j=1}^n \omega_{ij}$
    \State Calculate Laplace matrix $L=W-D$
    \State Compute the eigenvectors $\mathcal{U}=\{u_1,...,u_n\}$ and eigenvalues $\{\lambda_1,...,\lambda_n\}$ from $L$
    \State Sort eigenvectors $\mathcal{U}$ based on eigenvalues 
    \State Determine the cluster numbers $k$ based on $\lambda_{1,...,k}\leq \theta$
    \State Construct key matrix $\mathcal{K}=\{u_1,...,u_k\}$, and get $y_i \in \mathcal{R}^k$ from $i$-th row from $\mathcal{K}$
    \State Cluster points $(y_i)_{i=1,...,n}$ into $k$ clusters with $k$-means.
\end{algorithmic}
\end{algorithm}

\subsection{Incremental Merging}
\label{sec:merging}
Recall that in Figure.~\ref{fig:pipeline}, the data from different agents will stream to the AutoMerge server in random order.
/added{To achieve stable and accurate incremental merging, the AutoMerge operations contain the following three steps:
\begin{itemize}
    \item \textbf{Step1:} When each agent $v_i$ streams their observations and local place descriptors back to the server, AutoMerge will automatically detect the potential overlaps based on our Adaptive loop closure detection mechanism as stated in Section.~\ref{sec:lcd},
    and parallel estimate the overlaps' transformation via GICP~\cite{GICP} based point cloud alignment.
    \item \textbf{Step2:} As shown in Fig.~\ref{fig:inc_merge}, when new observation for agent $v_{i}$ received, AutoMerge will automatically estimate corresponding weightings $\omega_{ij}, i\neq j$ between $v_{i}$ and $v_j\in \bar{v}_i$; 
    when new overlaps are observed for existing agents, the previous weak connection ($\omega_{2,8}$) is further enhanced.
    \item \textbf{Step3:} Given the received agent lists $V_N=\{v_1,...,v_{N}\}$ and their relative overlap weighting $\omega_{ij}$, the system applies the graph clustering based on Section.~\ref{sec:spectral} to generated individual stable sub-groups $A_M=\{A_1,..., A_m\}$.
    \item \textbf{Step4:} Based on updated graphs, AutoMerge applies the standard back-end graph optimization for each sub-graph in $A_M$.
    The optimized position is sent back to all the agents for global pose estimation. Then go back to \textbf{Step1}.
\end{itemize}
In the above operations, the core of AutoMerge merging is triggered by Step2 and Step3 especially, which can adaptively fuse new observations into the global mapping ignoring their relative data streaming order.
Therefore, AutoMerge can transform the current offline high-resolution mapping into an incremental version.}
\deleted{This procedure will require the loop closure detection to automatically find the potential overlaps between different agents, ignoring data-stream order.
In the AutoMerge server system, each agent has its own identity (Agent-ID).
As shown in Fig.~\ref{fig:inc_merge}, based on multi-agent clustering stated in Section.~\ref{sec:spectral}, the received agent lists $V=\{v_1,...,v_10\}$ can be clustered into $2$ sub-groups $\{A_1, A_2\}$ based on their existing connections.
When new observation for agent $v_{i}$ received, AutoMerge will automatically estimate corresponding weightings $\omega_{ij}, i\neq j$ between $v_{i}$ and $v_j\in \bar{v}_i$; 
when new overlaps are observed for existing agents, previous weak connection ($\omega_{2,8}$) is further enhanced.
And based on updated global graphs, AutoMerge will merge original sub-groups into a joint graph.
During the merging procedure, all of the different sub-graph are optimized through self-contained individual graph optimization.}


==> doc_review/method/system.tex <==
\section{SYSTEM OVERVIEW}
As shown in Fig.~\ref{fig:pipeline}, AutoMerge provides an automatic map merging system for the large-scale single-/multi- agent mapping task\added{s}.
Each agent is equipped with a LiDAR mapping module to enable \added{the }self-maintained sub-map generation and odometry estimation.
The AutoMerge system consists of three modules: 1) fusion-enhanced place descriptor extraction, 2) an adaptive data-association mechanism to provide high accuracy and recall for segment-wise place retrievals, and 3) a partially decentralized system to provide centralized map merging and single agent self-localization in the world frame.

\added{\textbf{Problem Formulation}
\label{sec:formulation}
We define the trajectory list as $V_N=\{v_1,v_2,...,v_n\}$, each agent starts from the random position in the unknown map without initial coordinate knowledge and uploads the local odometry and 3D observations to the server incrementally.
And please note that the data streaming order of $V_N$ is random and in an incremental manner.
We assume can estimate a confidence score $\omega_{ij}\sim [0,1]$ based on the overlap between two trajectories $v_i$ and $v_j$.
The task of AutoMerge is to generate the accurate global maps $M_{global}$ combined by locally connected sub-groups $A_M=\{A_1,...,A_m\}$, based on the data stream from the trajectory list $V_N$ and their relative confidence matrix $\Omega_{N\times N}=\{\omega_{11},..., \omega_{1n};...;\omega_{n1},...,\omega_{NN}\}$, ignoring the order and completeness of the reserved data.}

\textbf{Fusion-enhanced Descriptor:}
\label{sec:decent_local}
Each agent runs the decentralized mapping sub-system as an extension of LiDAR-inertial odometry estimation~\cite{LOAM:zhang2014loam}, which also provides a sub-map extraction module for onboard adaptive descriptor extraction.
Such a descriptor has the following advantages:
1) it is translation-invariant due to the local translation-equivalent property of 3D point-clouds~\cite{adafusion}, 2) it is orientation-invariant due to the rotation-equivalent property of spherical harmonics~\cite{spherevlad}, and 3) it is light-weight compared to the original raw sub-maps.
Thus, a single agent can provide paired viewpoint-invariant place descriptors and ego-motion to the AutoMerge server system through lower bandwidth communication.

\textbf{Adaptive Loop Closure Detection:}
Spurious loop closures are frequent in environments with repetitive appearances, such as long streets.
On the one hand, false positive place retrievals may easily break the global optimization system, and ideally $100\%$ accuracy can avoid these optimization failures for large-scale mapping.
On the other hand, low recalls can provide partial data association, which will affect global optimization performance.
Hybrid loop closure detection takes advantage of sequence matching to provide continuous true positive retrievals over long overlaps, and RANSAC-based single frame detection for local overlaps. 
By \replaced{analyzing}{analysing} the feature correlation between segments, we can balance the place retrievals from sequence-/single- frame matching to provide accurate retrievals for offline/online LCD.

\textbf{Incremental Merging:}
Traditional centralized map merging~\cite{Merge:LAMP} is usually reliant on initial relative odometry estimation and geometry-based point cloud registration.
% Such methods are very sensitive to odometry drifts.
\deleted{Such methods are very sensitive to odometry drifts.}
In contrast, AutoMerge \replaced{uses}{can use} the paired place descriptors and ego motions of each agent to capitalize on loop closure opportunities (high accuracy and recall) for correction, despite a large amount of odometric drift.
Using this hybrid loop closure detection method, AutoMerge performs a rough centralized global map optimization\deleted{ \textbf{GO}}.
\added{Given the obtained information $V_N$ and their relative confidence matrix $\Omega_{N\times N}$, AutoMerge utilizes the spectral clustering method to adaptively merge different trajectories into different sub-groups $A_M$.
And our system can make each individual sub-group is well connected for the trajectories within, and no wrong matches are built between different sub-groups.
This mechanism ensure the incremental map merging ability, when the data stream of different agent in the list $V_N$ come with different time-order or completeness.}
\deleted{In the \textbf{Rough Merge} step, AutoMerge picks one segment as the root node and transforms other segments onto the existing nodes based on their keyframe associations and ICP-based local map alignments. 
The disadvantage of descriptor-based data association is the low accuracy since it ignores the true transformation between segments. 
In the \textbf{Refine Merge} step, AutoMerge calculates the accurate transform via geometry-based point cloud registration for all paired overlaps and utilizes a factor graph to refine the final merged results. 
After merging, each agent can optimize its localization, \textbf{LO}, through \textbf{GO} and its own odometry estimation.
In offline map merging, AutoMerge can detect all of the potential matches between all of the segments, and directly merge sub-maps into a global map along high-confidence overlaps.
In online map merging, the AutoMerge server can incrementally accumulate the key-frames and corresponding poses and merges segments with strong connections.}
% In the \textbf{Rough Merge} step, AutoMerge picks one segment as the root node and transforms other segments onto the existing nodes based on their keyframe associations.
% This step can extract the potential match segments between two trajectories, and use such segments to achieve rough alignment for the two trajectories via the ICP-based alignments, which treat one trajectory as one point cloud.
% The disadvantage of descriptor-based data association is the low accuracy since it ignores the true transformation between segments.
% In the \textbf{Refine Merge} step, AutoMerge calculates the accurate transform via geometry-based point cloud registration for all paired overlaps and utilizes a factor graph to refine the final merged results. 
% After merging, each agent can optimize its localization, \textbf{LO}, through \textbf{GO} and its own odometry estimation.
% In offline map merging, AutoMerge can detect all of the potential matches between all of the segments, and directly merge sub-maps into a global map along high-confidence overlaps.
% In online map merging, the AutoMerge server can incrementally accumulate the key-frames and corresponding poses and merges segments with strong connections.


==> doc_review/related.tex <==
\section{Related Works}
\label{sec:related_works}

    Map merging is defined as reorganizing unordered sub-maps into one global and consistent map.
    Related works investigate map merging using different sensing modalities, including vision~\cite{kimera_multi}, sonar~\cite{multi_agent_sonar}, and LiDAR~\cite{Merge:LAMP}; LiDAR-based approaches have been widely applied in large-scale mapping due to their robustness to illumination changes and environmental conditions~\cite{VPR:SURVEY}.
    In this section, we mainly target the 3D map merging task, and investigate recent state-of-the-art approaches.
    We also briefly introduce the key techniques of 3D feature extraction and large-scale data association.

       \begin{table*} [htbp]
        \caption{Comparison of different map merging approaches.}
        \centering
        \begin{tabular}{|C{2.5cm}|C{2cm}|C{1.5cm}|C{2.5cm}|C{2cm}|C{2cm}|C{2.5cm}|}
            \hline
            \textbf{Method}
            & \textbf{Environments}
            & \textbf{Scale(km)}
            & \textbf{Single/Multi Robots}
            & \textbf{Offline}
            & \textbf{Online}
            & \textbf{Works Without Initialization}
            \\
            \hline
            LAMP~\cite{Merge:LAMP} & Subterranean & $\leq 2$ & Multi & & \checkmark & \\
            \hline
            Kimera-Multi~\cite{kimera_multi} & Outdoor & $\leq 2$ & Multi & & \checkmark & \\
            \hline
            Multi-SLAM~\cite{multi_agent_fast_slam} & Indoor & $\leq 0.5$ & Multi & & \checkmark & \\
            \hline
            RTAB-Map~\cite{rtabmap} & Indoor & $\leq 0.5$ & Single & & \checkmark & \\
            \hline
            SegMap~\cite{segmap} & Outdoor & $\sim 10$ & Single & \checkmark & & \checkmark \\
            \hline
            AutoMerge (ours) & Outdoor & $\geq 100$ & Single/Multi & \checkmark & \checkmark & \checkmark\\
            \hline
        \end{tabular}
        \label{tab:CorrelationAveraging}
    \end{table*}

\subsection{Large-scale Map Merging}
\label{sec:map_merging}
    We review the literature on 3D SLAM systems for large-scale mapping, and refer the reader to~\cite{SLAM3D_survey} for a broader survey on 3D mapping.
    In general, 3D map merging is considered as map integration of different sub-maps with and without initial estimation.
    These 3D maps are typically represented as 3D point clouds, occupancy grids~\cite{octomap}, or 3D meshes~\cite{kimera}.
    % For 3D point cloud based
    Point cloud-based methods~\cite{Merge:LAMP}, mainly rely on geometric-based point cloud registration (such as ~\cite{icp,GICP}) to convert a point cloud into local 3D maps.
    The performance of the point-based approach is highly dependent on the robustness of 3D geometric features.
    % For occupancy based
    In most cases, map merging algorithms operate using occupancy grids~\cite{multi_agent_fast_slam}, which are obtained by selecting a plane, e.g. a ground plane in the case of a wheeled robot.
    However, the simple representations in occupancy-based approaches cannot satisfy current requirements for long-term 3D navigation tasks.
    Kimera~\cite{kimera}, a mesh-based method, provides a deformation graph model to merge 3D meshes between different agents.
    This approach can ensure 3D mesh consistency when used in multi-agent distributed mapping~\cite{kimera_multi}.
    % Common Limitation
    Most of the 3D map merging methods mentioned above are based on the assumptions that either all the sub-maps have the same initial pose~\cite{Merge:LAMP} or the mapping zones are restricted to a relatively small area~\cite{kimera_multi}.
    RTAB-Map \cite{rtabmap} is able to perform multi-session mapping using visual appearance-based LCD methods, through which a single robot can map separate areas in different sessions without giving relative initial poses between them.
    SegMap~\cite{segmap} can provide street block-like global map merging, but its data association is highly reliant on the segmentation of distinguishable semantic objects, which is hard to satisfy in a city-scale or campus-scale map merging task.
    In all the above methods, the success of large-scale map merging is highly reliant on accurate data association between different segments.
    However, accurate place feature extraction and data association are difficult to guarantee, especially for large-scale map merging. 
    In Table.~\ref{tab:CorrelationAveraging}, we compare AutoMerge with existing merging methods; our method is able to merge large-scale maps for single- and multi-agent scenarios, both offline and online, and without initialization.
    
\subsection{Place Feature Extraction}
\label{sec:place_feature}
    Place feature extraction is the core module for providing accurate data association for map merging.
    LiDAR is the preferred sensor used for place feature extraction, since LiDAR inputs are inherently invariant to illumination changes.
    % Point-based 3D place recognition
    A representative example of the point-based approach to place feature extraction is PointNetVLAD~\cite{PR:pointnetvlad}; in this work, Mikaela~\textit{et al} utilized PointNet~\cite{feature:pointnet} to extract local features and cluster them into a global place descriptor via the deep vector of locally aggregated descriptors (VLAD)~\cite{NetVLAD}. 
    This work enables learning the 3D place features directly from a point cloud.
    But PointNetVLAD omits the inner connections between points, which will significantly reduce the localization accuracy under different viewpoints.
    Based on the extended 3D point feature extraction of PointNet++~\cite{pointnet++}, LPD-Net~\cite{liu2019lpd} takes both point cloud and handcrafted features as inputs and introduces a graph-based aggregation module to learn multi-scale spatial information.
    % Projection-based 3D place recognition
    On the other hand, Projection-based approach has also been widely applied in non-learning and learning-based methods.
    Non-learning based methods, such as distance and angle based features ESF~\cite{esf}, structure based Scan-Context~\cite{cohen2018spherical,lpr:scan++}, and histogram-based features SHOT~\cite{shot}, have shown accurate recognition ability in city-scale environments, but are sensitive to large translation difference.
    \cite{lpr:stable} utilizes adversarial feature learning to improve the generalization ability of projection methods for local translation differences.
    In our previous work SphereVLAD~\cite{seqspherevlad}, we use spherical harmonics to obtain a viewpoint-invariant descriptor for 3D place recognition.
    In OverlapNet~\cite{PR:overlapnet}, the authors utilize a deep neural network to exploit different cues from LiDAR to estimate loop closures and the relative orientations.
    % Transformer enhanced place recognition
    Hui~\textit{et al.}~\cite{lpr:Point-Transformer} introduced a pyramid point cloud transformer network, based on the recent development of attention networks~\cite{attention_all_your_need}; this work improves the place recognition ability for PointNetVLAD. Ma~\textit{et al.}~\cite{lpr:overlaptransformer} extend the loop closure detection ability of OverlapNet with an additional transformer module.
    In our previous work, FusionVLAD~\cite{fusionvlad}, we proposed a deep fusion network integrating different perspectives to learn features that are resistant to translation/orientation differences.

\subsection{Large-scale Data Association}
\label{sec:data_association}
    Data association is critical for estimating the single and inter-connections between sub-maps in the multi-agent map merging task.
    In current SLAM frameworks~\cite{SLAM3D_survey}, robots utilize a combination of global descriptors (e.g., bag-of-words vectors~\cite{VPR:DBOW2} and learned full-image descriptors~\cite{VLAD}) to find the overlaps between different sub-maps. 
    However, single scans may include measurement noise, especially in large-scale city environments~\cite{DATASET:KITTI}, which can cause incorrect matches between different segments.
    SeqSLAM~\cite{2012SeqSLAM} provides a sequence-based place recognition method, which can improve recognition accuracy using the difference of residuals of a sequence of observations under changing environmental conditions.
    In our previous work~\cite{spherevlad}, we integrated a sequence-matching method with our SphereVLAD to provide viewpoint-invariant place recognition ability under changing 3D environments.
    Recently, Shan~\textit{et al.}~\cite{lpr:ransac} provided a RANSAC-based data association method to remove outliers in data association.
    However, most of the above methods are focused on single-agent inner data association, but few show promising results for large-scale multi-agent map merging tasks, where the may exist significant perspective and appearance differences between observations.

